Approximation Algorithms for Smallest Intersecting Balls

We study a general smallest intersecting ball problem and its soft-margin variant in high-dimensional Euclidean spaces for input objects that are compact and convex. These two problems link and unify a series of fundamental problems in computational geometry and machine learning, including smallest enclosing ball, polytope distance, intersection radius, $\ell_1$-loss support vector machine, $\ell_1$-loss support vector data description, and so on. Leveraging our novel framework for solving zero-sum games over symmetric cones, we propose general approximation algorithms for the two problems, where implementation details are presented for specific inputs of convex polytopes, reduced polytopes, axis-aligned bounding boxes, balls, and ellipsoids. For most of these inputs, our algorithms are the first results in high-dimensional spaces, and also the first approximation methods. Experimental results show that our algorithms can solve large-scale input instances efficiently.

==> paper/omitted-proofs.tex <==

\subsection{Proof of Proposition~\ref{prop:sib_general}}\label{sec:sib_general_prop_proof}



\subsection{Proof of Theorem~\ref{thm:sib_general_opt}}\label{sec:sib_general_opt_proof}



\subsection{Proof of Proposition~\ref{prop:soft_sib}}\label{sec:soft_sib_prop_proof}





\subsection{Proof of Theorem~\ref{thm:soft_sib_opt}}\label{sec:soft_sib_opt_proof}





==> paper/preamble.tex <==
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{amsfonts}
\usepackage{bm}
\usepackage{bbm}
\usepackage{ctable}
\usepackage{enumerate}
\usepackage{fullpage}
\usepackage{graphicx}
\usepackage{hyperref}
\usepackage{import}
\usepackage{lipsum}
\usepackage{lineno}
\usepackage{ltexpprt}
\usepackage{multirow}
\usepackage{multicol}
\usepackage{psfrag}
\usepackage{titlesec}
\usepackage{xcolor}

\usepackage[shortlabels]{enumitem}
\usepackage[square,numbers]{natbib}
\usepackage[noabbrev, capitalize]{cleveref}
\usepackage[cal=boondoxo]{mathalfa}

\bibliographystyle{plainnat}

\DeclareFontFamily{U}{FdSymbolA}{}
\DeclareFontShape{U}{FdSymbolA}{m}{n}{<-> s * [1] FdSymbolA-Book}{}
\DeclareFontShape{U}{FdSymbolA}{m}{b}{<-> s * [1] FdSymbolA-Medium}{}
\DeclareSymbolFont{fdsymbols}{U}{FdSymbolA}{m}{n}
\SetSymbolFont{fdsymbols}{bold}{U}{FdSymbolA}{m}{b}
\DeclareMathSymbol{\bdiamond}{\mathbin}{fdsymbols}{130}


\DeclareMathOperator*{\redpoly}{{\bf redcvx}}
\DeclareMathOperator*{\conv}{{\bf conv}}
\DeclareMathOperator*{\dist}{{\bf dist}}
\DeclareMathOperator*{\bary}{{\bf bary}}
\DeclareMathOperator*{\argmax}{argmax}
\DeclareMathOperator*{\argmin}{argmin}
\DeclareMathOperator*{\subto}{s.t.}
\newcommand{\Oplus}{\ensuremath{\vcenter{\hbox{\scalebox{1.2}{$\oplus$}}}}}
\newcommand{\medcap}{\ensuremath{\vcenter{\hbox{\scalebox{1.2}{$\cap$}}}}}
\DeclareMathOperator*{\cproduct}{\operatorname*{\Oplus}}


\newcommand{\TODO}[1]{{\em\color{violet} TODO: {#1}}}
\newcommand{\TOOD}{\TODO}
\newcommand{\JQ}[1]{{\em\color{purple} (Jiaqi: {#1})}}
\newcommand{\OPT}{{\sf OPT}}
\newcommand{\eps}{\varepsilon}
\newcommand{\Prb}{\mathrm{Pr}}
\newcommand{\Exp}{\mathbbm{E}}
\newcommand{\Tr}{\mathbf{tr}}

\newcommand{\mm}[1]{{\boldsymbol{#1}}}
\newcommand{\bb}[1]{\mathbbm{#1}}
\newcommand{\cc}[1]{\mathcal{#1}}
\newcommand{\xt}[2]{{#1}^{(#2)}}
\newcommand{\eigen}[2]{\lambda_{#1}({#2})}
\newcommand{\eigenval}[2]{\lambda_{#1}({#2})}
\newcommand{\inprod}[2]{{\langle{#1}, {#2}\rangle}}
\newcommand{\mmexp}{\mathbf{exp}}
\newcommand{\mmint}{\mathbf{int}}
\newcommand{\mmdiag}{\mathbf{diag}}

\newcommand{\bA}{\bb{A}}
\newcommand{\bB}{\bb{B}}
\newcommand{\bC}{\bb{C}}
\newcommand{\bD}{\bb{D}}
\newcommand{\bE}{\bb{E}}
\newcommand{\bF}{\bb{F}}
\newcommand{\bG}{\bb{G}}
\newcommand{\bH}{\bb{H}}
\newcommand{\bI}{\bb{I}}
\newcommand{\bJ}{\bb{J}}
\newcommand{\bK}{\bb{K}}
\newcommand{\bL}{\bb{L}}
\newcommand{\bM}{\bb{M}}
\newcommand{\bN}{\bb{N}}
\newcommand{\bO}{\bb{O}}
\newcommand{\bP}{\bb{P}}
\newcommand{\bQ}{\bb{Q}}
\newcommand{\bR}{\bb{R}}
\newcommand{\bS}{\bb{S}}
\newcommand{\bT}{\bb{T}}
\newcommand{\bU}{\bb{U}}
\newcommand{\bV}{\bb{V}}
\newcommand{\bW}{\bb{W}}
\newcommand{\bX}{\bb{X}}
\newcommand{\bY}{\bb{Y}}
\newcommand{\bZ}{\bb{Z}}

\newcommand{\mma}{\mm{a}}
\newcommand{\mmb}{\mm{b}}
\newcommand{\mmc}{\mm{c}}
\newcommand{\mmd}{\mm{d}}
\newcommand{\mme}{\mm{e}}
\newcommand{\mmf}{\mm{f}}
\newcommand{\mmg}{\mm{g}}
\newcommand{\mmh}{\mm{h}}
\newcommand{\mmi}{\mm{i}}
\newcommand{\mmj}{\mm{j}}
\newcommand{\mmk}{\mm{k}}
\newcommand{\mml}{\mm{l}}
\newcommand{\mmm}{\mm{m}}
\newcommand{\mmn}{\mm{n}}
\newcommand{\mmo}{\mm{o}}
\newcommand{\mmp}{\mm{p}}
\newcommand{\mmq}{\mm{q}}
\newcommand{\mmr}{\mm{r}}
\newcommand{\mms}{\mm{s}}
\newcommand{\mmt}{\mm{t}}
\newcommand{\mmu}{\mm{u}}
\newcommand{\mmv}{\mm{v}}
\newcommand{\mmw}{\mm{w}}
\newcommand{\mmx}{\mm{x}}
\newcommand{\mmy}{\mm{y}}
\newcommand{\mmz}{\mm{z}}

\newcommand{\mmA}{\mm{A}}
\newcommand{\mmB}{\mm{B}}
\newcommand{\mmC}{\mm{C}}
\newcommand{\mmD}{\mm{D}}
\newcommand{\mmE}{\mm{E}}
\newcommand{\mmF}{\mm{F}}
\newcommand{\mmG}{\mm{G}}
\newcommand{\mmH}{\mm{H}}
\newcommand{\mmI}{\mm{I}}
\newcommand{\mmJ}{\mm{J}}
\newcommand{\mmK}{\mm{K}}
\newcommand{\mmL}{\mm{L}}
\newcommand{\mmM}{\mm{M}}
\newcommand{\mmN}{\mm{N}}
\newcommand{\mmO}{\mm{O}}
\newcommand{\mmP}{\mm{P}}
\newcommand{\mmQ}{\mm{Q}}
\newcommand{\mmR}{\mm{R}}
\newcommand{\mmS}{\mm{S}}
\newcommand{\mmT}{\mm{T}}
\newcommand{\mmU}{\mm{U}}
\newcommand{\mmV}{\mm{V}}
\newcommand{\mmW}{\mm{W}}
\newcommand{\mmX}{\mm{X}}
\newcommand{\mmY}{\mm{Y}}
\newcommand{\mmZ}{\mm{Z}}

\newcommand{\mmgamma}{{\boldsymbol{\gamma}}}
\newcommand{\mmlambda}{{\boldsymbol{\lambda}}}
\newcommand{\mmmu}{{\boldsymbol{\mu}}}
\newcommand{\mmxi}{{\boldsymbol{\xi}}}
\newcommand{\mmeta}{{\boldsymbol{\eta}}}
\newcommand{\mmpsi}{{\boldsymbol{\psi}}}
\newcommand{\mmone}{\mm{1}}
\newcommand{\mmzero}{\mm{0}}
\newcommand{\brmf}{{\rm\bf f}}


\newcommand{\psd}{\mathbb{S}^n}
\newcommand{\la}{\langle}
\newcommand{\ra}{\rangle}
\newcommand{\lp}{\left(}
\newcommand{\rp}{\right)}
\newcommand{\p}{\partial}
\newcommand{\sub}{\subseteq}
\newcommand{\lam}{\lambda}
\newcommand{\calf}{\mathcal{F}}
\newcommand{\cala}{\mathcal{A}}
\newcommand{\LRI}{\Longrightarrow}
\newcommand{\epsi}{\epsilon}


\newcommand{\face}{\triangleleft}
\newcommand{\R}{\mathbb{R}}
\newcommand{\C}{\mathbb{C}}
\newcommand{\T}{\mathcal{T}}
\newcommand{\V}{\mathcal{V}}
\newcommand{\RR}{\mathcal{R}}
\newcommand{\HH}{\mathcal{H}}
\newcommand{\U}{\mathcal{U}}
\newcommand{\M}{\mathcal{M}}

\newcommand{\tr}{\mathrm{tr}}

\newcommand{\mcx}{\mathcal{X}}
\newcommand{\mcl}{\mathcal{L}}

\newcommand{\mcy}{\mathcal{Y}}
\newcommand{\mcq}{\mathcal{Q}}
\newcommand{\gam}{\Gamma}

\newcommand{\elon}{\epsilon}
\newcommand{\empi}{P_{x^k}}
\newcommand{\tclass}{T^k_P}
\newcommand{\pdclass}{T^k_{P,\delta}}
\newcommand{\da}{\dagger}

\newcommand{\SOC}{{\rm SOC}}
\newcommand{\Unif}{{\rm Unif}}


\usepackage{enumerate}
\usepackage{mdframed}
\mdfdefinestyle{MyFrame}{%
    linecolor=black,
    outerlinewidth=2pt,
    innertopmargin=4pt,
    innerbottommargin=4pt,
    innerrightmargin=4pt,
    innerleftmargin=4pt,
        leftmargin = 4pt,
        rightmargin = 4pt
        }


\newcommand{\bfy}{\mathbb{y}}
\newcommand{\bfxi}{\mathbb{\xi}}
\newcommand{\bfu}{\mathbb{u}}
\newcommand{\sqt}{{1\over \sqrt{2}}}


\newcommand{\na}{\nabla}


\newcommand{\txi}{\tilde{\xi}}
\newcommand{\tu}{\tilde{u}}
\newcommand{\ty}{\tilde{y}}
\newcommand{\tp}{\tilde{p}}


\DeclareMathOperator{\expl}{{\bf exp}}

\def\bpm{\begin{pmatrix}}
\def\epm{\end{pmatrix}}
\def\bal{\begin{aligned}}
\def\eal{\end{aligned}}


\newcommand{\aff}{\mathrm{aff}}
\newcommand{\ca}{\mathcal{A}}
\newcommand{\cj}{\mathcal{J}}
\newcommand{\cq}{S_{\mathcal{J}}}

\newcommand{\sfT}{{\sf T}}


\newcommand{\lqqd}{L(\R^{q \times q},\R^d)}

\newcommand{\ba}{{a}}
\newcommand{\bc}{{c}}
\newcommand{\be}{{e}}
\newcommand{\bu}{{u}}
\newcommand{\bv}{{v}}
\newcommand{\bw}{{w}}
\newcommand{\bx}{{x}}
\newcommand{\by}{{y}}
\newcommand{\bz}{{z}}


\newcommand{\lj}{\langle}
\newcommand{\rj}{\rangle}
\newcommand{\tb}{b_k}


\newcommand{\bi}{\begin{itemize}}
\newcommand{\ei}{\end{itemize}}
\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}
\newcommand{\itr}{{\rm int}}
\newcommand{\ben}{\begin{enumerate}}
\newcommand{\een}{\end{enumerate}}


==> paper/sib_cvx.tex <==
Given a set of convex polytopes, we want to find a ball with the smallest radius that intersects all the polytopes. 
More formally,
let $\cc{V}_i, i = 1, \dots, n, n > 1$, be non-empty finite point sets in the Euclidean space $\bR^d$, where $\cc{V}_i$ consists of $m_i$ points, and let $\Omega_i = \conv(\cc{V}_i),\ \forall i \in [n]$, be the convex hull of the corresponding point sets. The SIB problem is to find a ball $B(\mmz, r)$ with the smallest radius $r \ge 0$ such that $B(\mmz, r) \cap \Omega_i \neq \varnothing,\ \forall i \in [n]$.
In general, the smallest intersecting ball may not be unique. 
For example, if $n=2$ and $\Omega_1, \Omega_2$ are parallel line segments with non-trivial projections to each other, then there are infinitely many balls that intersect both $\Omega_1$ and $\Omega_2$ with the smallest radius.
On the other hand, a smallest intersecting ball of $\Omega_i$'s always exists. 
This problem is studied by~\cite{sibtheory:NNS2012} for general convex sets in a Banach space (a complete normed vector space).

\begin{lemma}[Proposition 3.2 in \cite{sibtheory:NNS2012}]\label{oldlem:sib_existence}
Let $\Omega_i, i = 1,\dots, n$, be nonempty closed convex sets in a Banach space. Suppose there exists $i\in [n]$ such that $\Omega_i$ is bounded. Then a smallest intersecting ball of $\Omega_i$'s always exists.
\end{lemma}

Given a point set $\cc{V} = \{\mmv_1, \dots, \mmv_m\}$ in $\bR^d$, every point in $\conv(\cc{V})$ can be represented by a convex combination of the points in $\cc{V}$.
In other words,
$\conv(\cc{V}) = \big\{\sum_{j=1}^m q_j \mmv_j : \forall \mmq \in \Delta^{m-1}\big\}$,
where $\Delta^{m-1} = \{\mmq \in \bR^m_+ : \mmone^T \mmq = 1\}$ is a {\em simplex}.
For a given point $\mmp\in\conv(\cc{V})$, we say $\mmq$ is a {\em barycentric coordinate} of $\mmp$ if and only if $\sum_j q_j \mmv_j = \mmp$. 
When $\cc{V}$ is a general point set without further restrictions, the barycentric coordinate of a point may not be unique~\cite{barycentric:Warren2002}.
However, the uniqueness and construction of barycentric coordinates are not necessary for our algorithms.
In this paper we use $\bary(\mmp, \cc{V}) = \big\{\mmq\in\Delta^{m-1} : \sum_j q_j \mmv_j = \mmp\big\}$ to denote the set of all valid barycentric coordinates of $\mmp$.

For $i=1,\dots,n$, let $\mmV_i$ be a ${d\times m_i}$ matrix such that its $j$-th column corresponds to the $j$-th point in $\cc{V}_i$.
Then every point $\mmp\in\Omega_i$ can be represented as $\mmp=\mmV_i\mmq_i$, where $\mmq_i \in \bary(\mmp, \cc{V}_i)$ is a barycentric coordinate of~$\mmp$.
We model the SIB problem as the following optimization problem:
\beq\label{oldeq:sib_cvx_problem}
\begin{aligned}
    \underset{\mmz, \mmq_1, \dots, \mmq_n, r}{\text{minimize}} \quad &r\\
    \text{subject to}\quad & \| \mmz - \mmV_i \mmq_i \| \le r,\ \forall i\in [n],\\
    & \mmone^T \mmq_i = 1,\ \forall i \in [n], \\
    & \mmq_i \geq 0,\ \forall i \in [n].
\end{aligned}
\eeq

\begin{proposition}\label{oldprop:sib_cvx_prop}
Let $\cc{V}_i, i = 1, \dots, n$, be point sets in $\bR^d$, and let $\Omega_i = \conv(\cc{V}_i), \forall i \in [n]$.
\begin{enumerate}
    \item[$(i)$] $B(\mmz, r)$ is a smallest intersecting ball of $\Omega_i$'s if and only if there exists $(\mmq_1, \dots, \mmq_n)$ such that $(\mmz, \mmq_1, \dots, \mmq_n, r)$ is an optimal solution of problem~\eqref{eq:sib_cvx_problem}.
    \item[$(ii)$] Problem~\eqref{eq:sib_cvx_problem} is a convex program and a solution always exists.
    \item[$(iii)$] $B(\mmz, r)$ is a smallest intersecting ball of $\Omega_i$'s only if $\mmz \in \conv(\{\Omega_i\}_{i=1}^n)$.
\end{enumerate}
\end{proposition}

\begin{proof}
$(i)$
For $i=1,\dots, n$, let $\mmp_i$ be a point in $B(\mmz, r)\cap \Omega_i$. Since $B(\mmz, r)\cap \Omega_i\neq \varnothing, \forall i \in [n]$, such a point must exists. For $i=1,\dots,n$, let $\mmq_i\in \bary(\mmp_i, \cc{V}_i)$ be a barycentric coordinate of $\mmp_i$. Then,
\[
    \|\mmz - \mmV_i\mmq_i\| \le r, \: \mmone^T \mmq_i = 1\ \text{and}\ \mmq_i\ge 0, \quad \forall i\in [n].
\]
Thus $(\mmz, \mmq_1, \dots, \mmq_n, r)$ is a feasible solution of problem~\eqref{eq:sib_cvx_problem}. Assume by contradiction that problem~\eqref{eq:sib_cvx_problem} has a solution $(\mmz', \mmq_1', \dots, \mmq_n', r')$ such that $r' < r$. Then $B(\mmz', r')$ is a smaller intersecting ball of $\Omega_i$'s.

We now justify the converse. Let $(\mmz, \mmq_1, \dots, \mmq_n, r)$ be an optimal solution of~\eqref{eq:sib_cvx_problem}. Then,
\[
    B(\mmz, r) \cap \Omega_i \neq \varnothing,\: \forall i \in [n].
\]
Assume by contradiction that there exists $\mmz'\in \bR^d$ and $r'< r$ such that $B(\mmz', r')\cap \Omega_i \neq \varnothing$ for all $i\in [n]$. Then there exists $(\mmq_1', \dots, \mmq_n')$ such that $(\mmz', \mmq_1', \dots, \mmq_n', r')$ is a feasible solution of~\eqref{eq:sib_cvx_problem} with a smaller objective value.


$(ii)$
For $i = 1, \dots, n$, define a function $\mmg_i : \bR^d \times \bR^{m_i} \times \bR \rightarrow \bR$ as follows:
\beq\label{oldeq:sib_cvx_constr}
\mmg_i(\mmz, \mmq_i, r) = \|\mmz - \mmV_i \mmq_i\| - r.
\eeq
Then the constraint $\|\mmz - \mmV_i\mmq_i\| \le r$ is equivalent to $\mmg_i(\mmz, \mmq_i, r) \le 0$.
Let $(\xt{\mmz}{1}, \xt{\mmq}{1}_i, \xt{r}{1})$ and $(\xt{\mmz}{2}, \xt{\mmq}{2}_i, \xt{r}{2})$ be any two points in the domain $\bR^d\times \bR^{m_i}\times \bR$.
Then for all $0\le t\le 1$, we have
\[\begin{aligned}
\hspace{10em}
&\mmg_i(t\xt{\mmz}{1} + (1 - t)\xt{\mmz}{2},\ t\xt{\mmq}{1}_i + (1 - t)\xt{\mmq}{2}_i,\ t\xt{r}{1} + (1 - t)\xt{r}{2})\\
=\:& \|t\xt{\mmz}{1} + (1 - t)\xt{\mmz}{2} - \mmV_i(t\xt{\mmq}{1}_i + (1 - t)\xt{\mmq}{2}_i) \| - (t\xt{r}{1} + (1 - t)\xt{r}{2}) &\\
=\:& \|t\xt{\mmz}{1} - t\mmV_i\xt{\mmq}{1}_i + (1 - t)\xt{\mmz}{2} - (1 - t)\mmV_i\xt{\mmq}{2}_i \| - t\xt{r}{1} - (1 - t)\xt{r}{2}\\
\le\: & t\|\xt{\mmz}{1} - \mmV_i\xt{\mmq}{1}_i\| + (1 - t)\|\xt{\mmz}{2} - \mmV_i\xt{\mmq}{2}_i \| - t\xt{r}{1} - (1 - t)\xt{r}{2} &\text{(Triangle inequality)}\\
=\: & t \mmg_i(\xt{\mmz}{1}, \xt{\mmq}{1}_i, \xt{r}{1}) + (1-t) \mmg_i(\xt{\mmz}{2}, \xt{\mmq}{2}_i, \xt{r}{2}),
\end{aligned}\]
which proves that function~\eqref{eq:sib_cvx_constr} is convex. Since the objective is linear and all other constraints are linear, problem~\eqref{eq:sib_cvx_problem} is a convex program.
The existence of a solution follows immediately from $(i)$ and Lemma~\ref{lem:sib_existence}.


$(iii)$
Let $\cc{D}$ be the convex hull $\conv(\{\Omega_i\}_{i=1}^n)$. Assume there exists a smalleset intersecting ball $B(\mmz, r)$ such that $\mmz\notin \cc{D}$. 
Let $\mmz' = \Pi(\mmz, \cc{D})$ be the Euclidean projection from $\mmz$ to $\cc{D}$. Thus $\|\mmz - \mmz'\| > 0$. For $i = 1, \dots, n$, let $\mmp_i$ be any point in $B(\mmz, r) \cap \Omega_i$. Then,
\[
\|\mmp_i - \mmz\|^2 = \|\mmp_i - \mmz' + \mmz' - \mmz\|^2 = \|\mmp_i - \mmz'\|^2 + \|\mmz' - \mmz\|^2 + 2\inprod{\mmp_i - \mmz'}{\mmz' - \mmz}.
\]
By the projection theorem~\cite[Theorem 9.8]{projtheory:Beck2014}, for every $\mmp \in \cc{D}$, $\inprod{\mmp - \mmz'}{\mmz' - \mmz}\ge 0$. Thus for each $i\in [n]$, we have
\[
    \|\mmp_i - \mmz'\|^2 < \|\mmp - \mmz'\|^2 + \|\mmz' - \mmz\|^2 + 2\inprod{\mmp_i - \mmz'}{\mmz' - \mmz} = \|\mmp_i - \mmz\|^2 \le r^2.
\]
Let $r' = \max_{i\in [n]} \|\mmp_i - \mmz'\|$.
Then the ball $B(\mmz', r')$ intersects all polytopes with the radius $r' < r$,
which is a contradictory result.
\end{proof}

Let $r^* > 0$ be the optimal value of problem~\eqref{eq:sib_cvx_problem} and $\eps>0$ be an error parameter. We say $(\mmz, \mmq_1, \dots, \mmq_n, r)$ is a $(1+\eps)$-approximate solution of~\eqref{eq:sib_cvx_problem} if it is feasible and $r\le (1+\eps)r^*$.
To find a $(1+\eps)$-approximate solution, we first consider a decision version of this problem. 
Given $\hat{r} > 0$, we want to either determine $\hat{r} < r^*$ or verify that $(1+\eps)\hat{r}\ge r^*$.
For the latter case, we find a solution of~\eqref{eq:sib_cvx_problem} with value at most $(1+\eps)\hat{r}$. We call this decision problem a {\em feasibility test problem} (FTP):
\begin{flalign}\label{oldeq:sib_cvx_ftp}
&\quad
\begin{aligned}
    &\text{\em Given $\hat{r} > 0$, find $\mmz, \mmq_1, \dots, \mmq_n, r$ such that}
\end{aligned}
\quad
\begin{aligned}
    &r \le (1+\eps)\hat{r},\\
    &\|\mmz - \mmV_i \mmq_i\| \le r, \ \forall i \in [n],\\
    &\mmq_i \in \Delta^{m_i - 1},\ \forall i \in [n],\\
    &\mmz \in \conv(\{\Omega_i\}_{i=1}^n).
\end{aligned}
&&
\end{flalign}
Let $D$ be the diameter of $\conv(\{\Omega_i\}_{i=1}^n)$.
It is easily seen that $r^* \le D$ because a ball centered at any input point with radius $D$ intersects all $\Omega_i$'s, and the problem of approximately solving~\eqref{eq:sib_cvx_problem} can be reduced to the problem of solving a sequence of FTPs via binary search.

\begin{theorem}\label{oldthm:sib_cvx_thm}
Let $M = \sum_{i=1}^n m_i$ and let $D$ be the diameter of the convex hull $\conv(\{\Omega_i\}_{i=1}^n)$.
Given $\hat{r} \in (0, D]$ and an error parameter $\eps \in (0, {4 D \over \hat{r}}]$, there is an iterative algorithm that solves the feasibility test problem~\eqref{eq:sib_cvx_ftp} in $O({D^2\log n \over \eps^2 \hat{r}^2})$ iterations, with a processing time of $O(Md)$ per iteration.
\end{theorem}
\begin{proof}
Observe that $(\mmz,\mmq_1,\dots,\mmq_n,r)$ is a feasible solution of~\eqref{eq:sib_cvx_problem} only if it satisfies
\beq\label{oldeq:sib_cvx_soc_constr}
    \|\mmz - \mmV_i \mmq_i\| \le r,\ \forall i \in [n].
\eeq
By the characterization~\eqref{eq:soc_characterization} of second-order cones, the above condition can be interpreted as $(\mmz - \mmV_i\mmq_i, r) \in \cc{Q}^{d+1}$ for $i = 1, \dots, n$.
Let $\bU = \bR^d \times \bR^{m_1}\times\dots \times \bR^{m_n} \times \bR$, and let $\brmf : \bU \rightarrow \bV$ be the linear map:
\[
    \brmf(\mmz, \mmq_1, \dots, \mmq_n, r) := \cproduct_{i=1}^n (\mmz - \mmV_i\mmq_i, r).
\]
Then the condition~\eqref{eq:sib_cvx_soc_constr} is equivalent to $\brmf(\mmz, \mmq_1, \dots, \mmq_n, r) \in \cc{C}$, where $\cc{C}$ is the product cone defined in~\eqref{eq:product_cone_defn}. Let $\cc{B} = \{\mmy\in\cc{C} : \Tr(\mmy) = 1\}$. By self-duality of $\cc{C}$, we know that $\brmf(\mmz,\mmq_1,\dots,\mmq_n,r)\in\cc{C}$ only if
\beq\label{oldeq:sib_cvx_innner_product}
   \brmf(\mmz,\mmq_1,\dots,\mmq_n,r) \bdiamond \mmy \ge 0,\ \forall \mmy \in \cc{B}.
\eeq


On the other hand, from the problem definition and Proposition~\ref{prop:sib_cvx_prop}, we know that $(\mmz^*, \mmq^*_1, \dots, \mmq^*_n, r^*)\in \bU$ is an optimal solution of~\eqref{eq:sib_cvx_problem} only if $\mmz^*\in \conv(\{\Omega_i\}_{i=1}^n)$ and $\mmq^*_i\in \Delta^{m_i - 1},\ \forall i \in [n]$.
Furthermore, if $\hat{r} \ge r^*$, we know that any optimal solution $(\mmz^*, \mmq^*_1, \dots, \mmq^*_n, r^*)$ must be in the convex set
\[
    \cc{A} = \Big\{(\mmz, \mmq_1,\dots,\mmq_n, r) \in \bU : \mmz\in\conv(\{\Omega_i\}_{i=1}^n),\ \mmq_i \in \Delta^{m_i - 1}, \forall i\in [n],\ r \le \hat{r} \Big\}.
\]

Let $\mmx = (\mmz, \mmq_1, \dots, \mmq_n, r)$ and let $\cc{O}^* \subseteq \bU$ be the set of all optimal solutions of~\eqref{eq:sib_cvx_problem}.
From~\eqref{eq:sib_cvx_innner_product} we know that $\min_{\mmy \in \cc{B}}\ \brmf(\mmx)\bdiamond \mmy \ge 0,\ \forall \mmx \in \cc{O}^*$.
If $\hat{r} \ge r^*$, then $\cc{O}^*\subseteq \cc{A}$ and consequently
\beq
    \max_{\mmx \in \cc{A}} \min_{\mmy\in\cc{B}} \ \brmf(\mmx) \bdiamond \mmy \ge 0,
\eeq
which means the value $\lambda^*$ of the zero-sum game with $\cc{A}$ and $\brmf$ defined as above is nonnegative.
Assume an {\sc Oracle} with width $\rho$ that provides the best response $\mmx\in \cc{A}$ to every $\mmy\in\cc{B}$.
We employ the algorithm described in Theorem~\ref{thm:zero-sum_game} to solve the zero-sum game up to an additive error $\eps\hat{r} / \sqrt{2}$.
During the process of this algorithm, if there is certain round $t$ such that $\max_{\mmx\in\cc{A}}\ \brmf(\mmx)\bdiamond\xt{\mmy}{t} < 0$, then $\lambda^* < 0$ and $\cc{O}^* \nsubseteq \cc{A}$. In which case we terminate the algorithm and conclude that $\hat{r} < r^*$.
Conversely, if we have $\brmf(\xt{\mmx}{t})\bdiamond \xt{\mmy}{t} \ge 0$ for all $t = 1, \dots, T$, then $\sum_{t=1}^T \brmf(\xt{\mmx}{t})\bdiamond \xt{\mmy}{t} \ge 0$ and inequality~\eqref{eq:zero-sum_game_eigenvalue} implies $\lambda_{\min}\big(\brmf(\tilde{\mmx})\big) + \eps\hat{r} / \sqrt{2} \ge 0$. Let $\tilde{\mmx} = (\tilde{\mmz}, \tilde{\mmq}_1, \dots, \tilde{\mmq}_n, \tilde{r})$. Then $\brmf(\tilde{\mmx}) = \cproduct_{i=1}^n (\tilde{\mmz} - \mmV_i \tilde{\mmq}_i, \tilde{r})$ and 
\[\begin{aligned}
    \lambda_{\min}\big(\cproduct_{i=1}^n (\tilde{\mmz} - \mmV_i \tilde{\mmq}_i, \tilde{r}) \big) + {\eps \hat{r} \over \sqrt{2}} \ge 0 
    \ \Longrightarrow \ 
    \cproduct_{i=1}^n (\tilde{\mmz} - \mmV_i \tilde{\mmq}_i, \tilde{r}) + {\eps \hat{r} \over \sqrt{2}} \mme \in \cc{C}
    \ \Longrightarrow \ 
    \cproduct_{i=1}^n (\tilde{\mmz} - \mmV_i \tilde{\mmq}_i, \tilde{r} + \eps\hat{r}) \in \cc{C}.
\end{aligned}\]
Since $\tilde{\mmz}\in\conv(\{\Omega_i\}_{i=1}^n)$, $\tilde{\mmq}_i \in \Delta^{m_i - 1}, \forall i \in [n]$, and $\tilde{r} + \eps\hat{r} \le (1 + \eps)\hat{r}$, we conclude that $(\tilde{\mmz}, \tilde{\mmq}_1, \dots, \tilde{\mmq}_n, \tilde{r} + \eps\hat{r})$ is a feasible solution of~\eqref{eq:sib_cvx_problem} with objective value at most $(1+\eps)\hat{r}$.

Now we have a closer look at the {\sc Oracle}. For any given $\mmy\in\cc{B}$, the {\sc Oracle} finds $\mmx = \argmax_{\mmx\in\cc{A}} \brmf(\mmx)\bdiamond\mmy$.
Let $\mmx = (\mmz, \mmq_1, \dots, \mmq_n, r)\in \bU$ and $\mmy = \cproduct_{i=1}^n (\bar{\mmy}_i, y_{i,0})\in\bV$, the problem can be formatted as:
\beq\label{oldeq:sib_cvx_oracle}
\begin{aligned}
    \underset{\mmz, \mmq_1, \dots, \mmq_n, r}{\rm maximize}\quad & \big(\sum_{i=1}^n \bar{\mmy}_i \big)^T \mmz - \sum_{i=1}^n (\bar{\mmy}_i^T \mmV_i ) \mmq_i + \big(\sum_{i=1}^n y_{i,0}\big)r\\
    {\rm subject\ to}\quad & \mmz\in\conv(\{\Omega_i\}_{i=1}^n),\\  
    & \mmq_i\in \Delta^{m_i - 1},\ \forall i \in [n],\\
    & r\le \hat{r}.
\end{aligned}
\eeq
Observe that the constraints on $\mmz$, each $\mmq_i$, and $r$ are independent. The problem can be decomposed into smaller problems and be solved individually. 
For $\mmz$, the problem is optimizing a linear function over the convex hull of all input 
points, which can be solved by computing the function value on each point.
For each $\mmq_i$, the problem is minimizing a linear function over a simplex, which can be solved by identifying the smallest entry in the vector $\bar{\mmy}_i^T \mmV_i$.
As for $r$, since $\sum_{i=1}^n y_{i,0}$ is a positive constant, the optimum is always achieved at $r = \hat{r}$.

Let $(\mmz, \mmq_1, \dots, \mmq_n, r)$ be a solution of problem~\eqref{eq:sib_cvx_oracle}.
The width $\rho$ of the {\sc Oracle} is an upperbound on the spectral norm of $\cproduct_{i=1}^n (\mmz - \mmV_i \mmq_i, r)$ over all possible inputs $\mmy\in\cc{B}$. Since $\mmq_i\in \Delta^{m_i - 1}$, the point $\mmV_i\mmq_i$ is in $\Omega_i$ and also $\conv(\{\Omega_i\}_{i=1}^n)$. Consequently, we have $\|\mmz - \mmV_i \mmq_i\| \le D,\ \forall i \in [n]$. Then,
\[\begin{aligned}
    \Big\|\cproduct_{i=1}^n (\mmz - \mmV_i \mmq_i, r)\Big\|_\spe 
    &= \max_{k\in [2n]}\ \Big|\lambda_{k}\big(\cproduct_{i=1}^n (\mmz - \mmV_i \mmq_i, r)\big) \Big| \\
    &\le \max_{i\in [n]}\ \|\mmz - \mmV_i\mmq_i\| + r\\
    &\le 2D.
\end{aligned}\]
For the last inequality, we used the fact that $r \le \hat{r} \le D$. Therefore, the {\sc Oracle} has a width of $2D$.
By our assumption that $\eps \le {4 D \over \hat{r}}$, the additive error $\eps\hat{r}/\sqrt{2}$ is at most $2\rho$ thus satisfies the condition in Theorem~\ref{thm:zero-sum_game}. The total number of iterations for approximating the zero-sum game
is $T = \lceil{32D^2 \ln(2n) \over \eps^2 \hat{r}^2}\rceil$. In each iteration, the algorithm calls the {\sc Oracle} and performs~\eqref{eq:game_update}, which takes $O(Md + nd) = O(Md)$ time.
\end{proof}

\begin{corollary}\label{oldcoro:sib_cvx_optimization}
Let $M = \sum_{i=1}^n m_i$ and let $D$ be the diameter of the convex hull $\conv(\{\Omega_i\}_{i=1}^n)$.
Let $r^* > 0$ be the optimal value of~\eqref{eq:sib_cvx_problem} and $R$ be the ratio $D\over r^*$. Given an error parameter $\eps>0$, a $(1+\eps)$-approximate solution of~\eqref{eq:sib_cvx_problem} can be computed in $O({R^2 Md \log n \over \eps^2})$ time.
\end{corollary}
\begin{proof}
{\em $(i)$ From FTP to optimization. } 
Let $L_0 = 0$, $U_0 = D$, $\hat{r}_1 = L_0 + {1\over 3}(U_0 - L_0)$ and $\eps_1 = {1\over 3\hat{r}_1}(U_0 - L_0)$. Employ the algorithm described in Theorem~\ref{thm:sib_cvx_thm} to solve an FTP with the parameters $\hat{r}_1$ and $\eps_1$ (note that ${\eps_1\hat{r}_1 \over \sqrt{2}} < 2\rho$). Then we can either conclude $\hat{r}_1 < r^*$ or find a solution $(\mmx, \mmq_1, \dots, \mmq_n, r)$ with $r \le (1+\eps_1)\hat{r}_1$. For the former case, we have
\[
    L_0 + {1\over 3}(U_0 - L_0) < r^* \le U_0,
\]
and for the latter case, we have
\[
    L_0 < r^* \le L_0 + {2\over 3}(U_0 - L_0).
\]
Set $L_1 = L_0 + {1\over 3}(U_0 - L_0),\ U_1 = U_0$ if the first case materializes and set $L_1 = L_0,\ U_1 = L_0 + {2\over 3}(U_0 - L_0)$ if the second case materializes. Both situations can be summarized as:
\[
    L_1 < r^* \le U_1,\ \text{where}\ (U_1 - L_1) = {2\over 3}(U_0 - L_0).
\]
Repeat this process by setting $\hat{r}_i = L_{i-1} + {1\over 3}(U_{i-1} - L_{i-1})$ and $\eps_i = {1\over 3\hat{r}_i}(U_{i-1} - L_{i-1})$ for $i\ge 2$, until the resultant $L_i$ and $U_i$ satisfy $U_i \le (1+\eps) L_i$. The last solution $(\mmx, \mmq_1, \dots, \mmq_n, r)$ we obtained from this process has value $r \le U_i \le (1+\eps)L_i < (1+\eps)r^*$, thus is an $(1 + \eps)$-approximate solution of~\eqref{eq:sib_cvx_problem}. For the parameters $\hat{r}_i$ and $\eps_i$, we have $\eps_i \hat{r}_i = {1\over 2}(U_i - L_i)$. Since $(U_i - L_i)$ shrinks by a constant fraction in each step, the quantity $\eps_i \hat{r}_i$ also decreases geometrically. The total running time will be dominated by the time for solving the last FTP (with the smallest $\eps_i \hat{r}_i = {1\over 2} \eps r^*$), which is $O({R^2 Md \log n \over \eps^2})$.

{\em $(ii)$ Working with unkown diameter. }
To make the algorithm work, it remains to determine the diameter $D$ of the convex hull $\conv(\{\Omega_i\}_{i=1}^n)$. The quantity $D$ serves two purposes in our algorithm. Firstly, it is an upperbound on the optimal value $r^*$; and secondly, it is related to the width of the {\sc Oracle}. 
There are many alternative approaches to obtain an initial upperbound on $r^*$. Instead of using the exact value of $D$, we can pick a point $\mmv_i$ in each $\Omega_i$ (in the current context, a point in each $\cc{V}_i$) and compute $E = \max_{i\in [n]} \|\mmv_i - \mmv_1\|$. It is clear that $E \le D$ and the ball $B(\mmv_1, E)$ intersects each $\Omega_i$. Thus $E$ is a suitable upperbound on $r^*$.
As for the width of the {\sc Oracle}, to ensure the algorithm's running time retains the same asymptotic order, it suffices to compute a constant approximation of $D$, which is straightforward in the current context. 
Nevertheless, it could be challenging when the convex sets $\Omega_i$'s become more complex (e.g.~when $\Omega_i$'s are boxes or ellipsoids). Here we introduce a general approach to address this scenario.

Recall that the width $\rho$ is an upperbound on $\|\brmf(\mmx)\|_\spe$, where $\mmx$ is any possible output of the {\sc Oracle}. The purpose of introducing $\rho$ is to ensure that the eigenvalues of $\brmf(\mmx) / \rho$ consistently fall within the range $[-1,1]$, thus all the inequalities in Theorem~\ref{thm:zero-sum_game} work appropriately.
Therefore, instead of bounding the spectral norm of $\brmf(\mmx)$ for all possible {\sc Oracle} outputs $\mmx$'s, it suffices to find an upperbound on $\|\brmf(\xt{\mmx}{t})\|_\spe$ for all $\xt{\mmx}{t}$'s that appear in the runtime. Let $\rho_1 = E$ be a foresight estimation on the upperbound. Run the algorithm described in $(i)$ with the estimated width $\rho_1$. Note that since we take $E$ as the initial $U_0$, we have ${\eps_1 \hat{r}_1 \over \sqrt{2}} < E < 2\rho_1$ and the condition on the error parameter in Theorem~\ref{thm:zero-sum_game} is always satisfied.
During the runtime, if there exists a certain iteration $t$ such that the value of $\|\brmf(\xt{\mmx}{t})\|_\spe$ exceeds $\rho_1$, we terminate the algorithm and set $\rho_2 = 2\rho_1$. Repeat this process by setting $\rho_i = 2\rho_{i-1}$ for $i\ge 2$, until we reach a value $\rho_{\rm final}$ so that the algorithm completes its full process and computes a $(1+\eps)$-approximate solution using the width $\rho_{\rm final}$. Since $\rho_1, \dots, \rho_{\rm final}$ form a geometric series, the total running time of this approach is dominated by $O({\rho_{\rm final}^2 Md \log n \over (\eps r^*)^2})$. Moreover, if $\rho_{\rm final} \neq \rho_1$, there must exists $\xt{\mmx}{t}$ such that $\|\brmf(\xt{\mmx}{t})\|_\spe > \rho_{\rm final} / 2$, in which case we have $\rho_{\rm final} / 2  < \rho$ and consequently $\rho_{\rm final} < 2\rho \le 4D$. Otherwise, if $\rho_{\rm final} = \rho_1 = E$, we have $\rho_{\rm final} \le D$. For both cases, the total running time is of the same asymptotic order as before.
\end{proof}

\begin{Remark}
\TODO{Implications on special cases}
\end{Remark}


==> paper/sib_variants.tex <==
\TODO{some intro}


\subsection{SIB of boxes}\label{oldsec:sib_box}
Let $\Omega_i,\ i = 1,\dots,n$, be non-empty axis-aligned bounding boxes (AABBs) in the Euclidean space $\bR^d$. To find a SIB of AABBs, we can represent each AABB as the convex hull of its vertices and apply the algorithm introduced in Section~\ref{sec:sib_cvx}.
However, since a $d$-dimentional AABB has $2^d$ vertices, this approach possesses a running time of $\widetilde{O}({R^2 2^d n d \over \eps^2})$ to compute a $(1+\eps)$-approxiamte solution.
Instead of viewing each AABB as a convex polytope, we represent an AABB by specifying the minimum and maximum coordinates in each dimension. Let $\mm{\ell}, \mmu$ be two vectors in $\bR^d$ such that $\mm{\ell} \le \mmu$. Then an AABB can be characterized as $\{\mmv\in \bR^d : \mm{\ell} \le \mmv \le \mmu\}$. With this characterization, we model the SIB problem for AABBs as the following optimization problem:
\beq\label{oldeq:sib_box_problem}
\begin{aligned}
    \underset{\mmz, \mmv_1, \dots, \mmv_n, r}{\text{minimize}} \quad &r\\
    \text{subject to}\quad & \|\mmz - \mmv_i\| \le r,\ \forall i \in [n],\\
    & \mm{\ell}_i \le \mmv_i \le \mmu_i,\ \forall i \in [n].
\end{aligned}
\eeq

\begin{proposition}\label{oldprop:sib_box_prop}
Let $\Omega_i, i = 1, \dots, n$, be axis-aligned bounding boxes in the Euclidean space $\bR^d$.
\begin{enumerate}
    \item[$(i)$] $B(\mmz, r)$ is a smallest intersecting ball of $\Omega_i$'s if and only if there exists $(\mmv_1, \dots, \mmv_n)$ such that $(\mmz, \mmv_1, \dots, \mmv_n, r)$ is an optimal solution of problem~\eqref{eq:sib_box_problem}.
    \item[$(ii)$] Problem~\eqref{eq:sib_box_problem} is a convex program and a solution always exists.
    \item[$(iii)$] $B(\mmz, r)$ is a smallest intersecting ball of $\Omega_i$'s only if $\mmz\in \conv(\{\Omega_i\}_{i=1}^n)$.
\end{enumerate}
\end{proposition}

The proof of Proposition~\ref{prop:sib_box_prop} is almost identical to Proposition~\ref{prop:sib_cvx_prop} so is omitted here.
Let $r^* > 0$ be the optimal value of problem~\eqref{eq:sib_box_problem} and $\eps>0$ be an error parameter. We say $(\mmz, \mmv_1, \dots, \mmv_n, r)$ is a $(1+\eps)$-approximate solution of~\eqref{eq:sib_box_problem} if it is feasible and $r\le (1+\eps)r^*$.
Similar to Section~\ref{sec:sib_cvx}, we first consider the feasibility test problem (FTP):
\begin{flalign}\label{oldeq:sib_box_ftp}
&\quad
\begin{aligned}
    &\text{\em Given $\hat{r} > 0$, find $\mmz, \mmv_1, \dots, \mmv_n, r$ such that}
\end{aligned}
\quad
\begin{aligned}
    &r \le (1+\eps)\hat{r},\\
    &\|\mmz - \mmv_i\| \le r, \ \forall i \in [n],\\
    &\mm{\ell}_i \le \mmv_i \le \mmu_i, \ \forall i \in [n],\\
    &\mmz \in \conv(\{\Omega_i\}_{i=1}^n).
\end{aligned}
&&
\end{flalign}
Let $D$ be the diameter of the convex hull $\conv(\{\Omega_i\}_{i=1}^n)$. It is easily seen that $r^* \le D$, and a FTP can be solved using an algorithm that is similar to the one introduced in Theorem~\ref{thm:sib_cvx_thm}.



\begin{theorem}\label{oldthm:sib_box}
Let $D$ be the diameter of the convex hull $\conv(\{\Omega_i\}_{i=1}^n)$. Given $\hat{r} \in (0, D]$ and an error parameter $\eps\in (0, {4 D \over \hat{r}}]$, there is an iterative algorithm that solves the feasibility test problem~\eqref{eq:sib_box_ftp} in $O({D^2 \log n \over \eps^2\hat{r}^2})$ iterations, with a processing time of $O(nd)$ per iteration.
\end{theorem}
\begin{proof}
Let $\bU = \bR^d \times \dots \times \bR^d \times \bR$, and let $\brmf : \bU \rightarrow \bV$ be a linear map defined as
\[
    \brmf(\mmz, \mmv_1, \dots, \mmv_n, r) = \cproduct_{i=1}^n (\mmz - \mmv_i, r).
\]
Then $\mmx = (\mmz, \mmv_1, \dots, \mmv_n, r)$ is a feasible solution of~\eqref{eq:sib_box_problem} only if $\brmf(\mmx) \in \cc{C}$, which implies $\brmf(\mmx) \bdiamond \mmy \ge 0, \ \forall \mmy \in \cc{B}$. Define the convex set
\[
    \cc{A} = \Big\{(\mmz, \mmv_1, \dots, \mmv_n, r) \in \bU : \mmz\in \conv(\{\Omega_i\}_{i=1}^n),\ \mm{\ell}_i \le \mmv_i \le \mmu_i, \forall i\in [n], \ r \le \hat{r} \Big\}.
\]
Let $\cc{O}^*\subseteq \bU$ be the set of all optimal solutions of~\eqref{eq:sib_box_problem}. From Proposition~\ref{prop:sib_box_prop}, we know that if $\hat{r} \ge r^*$, then $\cc{O}^* \subseteq \cc{A}$ and consequently
\[
    \max_{\mmx\in \cc{A}} \min_{\mmy\in \cc{B}}\ \brmf(\mmx) \bdiamond \mmy \ge 0.
\]

Assume an {\sc Oracle} with width $\rho$ that provides the best response $\mmx \in \cc{A}$ to every $\mmy \in \cc{B}$. Employ the algorithm described in Theorem~\ref{thm:zero-sum_game} to solve the zero-sum game up to an additive error $\eps\hat{r} / \sqrt{2}$. During the process of the algorithm, if there is a certain round $t$ such that $\max_{\mmx\in\cc{A}} \brmf(\mmx)\bdiamond \xt{\mmy}{t} < 0$, then the value of the game $\lambda^* < 0$ and $\cc{O}^* \nsubseteq \cc{A}$. In which case we terminate the algorithm and conclude that $\hat{r} < r^*$. 
Conversely, if we have $\brmf(\xt{\mmx}{t})\bdiamond \xt{\mmy}{t} \ge 0$ for all $t = 1, \dots, T$, then $\sum_{t=1}^T \brmf(\xt{\mmx}{t})\bdiamond \xt{\mmy}{t} \ge 0$ and inequality~\eqref{eq:zero-sum_game_eigenvalue} implies $\lambda_{\min}\big(\brmf(\tilde{\mmx})\big) + \eps\hat{r} / \sqrt{2} \ge 0$. 
Let $\tilde{\mmx} = (\tilde{\mmz}, \tilde{\mmv}_1, \dots, \tilde{\mmv}_n, \tilde{r})$. Then $\brmf(\tilde{\mmx}) = \cproduct_{i=1}^n (\tilde{\mmz} - \tilde{\mmv}_i, \tilde{r})$ and 
\[\begin{aligned}
    \lambda_{\min}\big(\cproduct_{i=1}^n (\tilde{\mmz} - \tilde{\mmv}_i, \tilde{r}) \big) + {\eps \hat{r} \over \sqrt{2}} \ge 0 
    \ \Longrightarrow \ 
    \cproduct_{i=1}^n (\tilde{\mmz} - \tilde{\mmv}_i, \tilde{r}) + {\eps \hat{r} \over \sqrt{2}} \mme \in \cc{C}
    \ \Longrightarrow \ 
    \cproduct_{i=1}^n (\tilde{\mmz} - \tilde{\mmv}_i, \tilde{r} + \eps\hat{r}) \in \cc{C}.
\end{aligned}\]
Since $\tilde{\mmv}_i \in \Omega_i$ and $\tilde{r} + \eps\hat{r} \le (1 + \eps)\hat{r}$, we conclude that $(\tilde{\mmz}, \tilde{\mmv}_1, \dots, \tilde{\mmv}_n, \tilde{r})$ is a feasible solution of problem~\eqref{eq:sib_box_problem} with objective value at most $(1+\eps) \hat{r}$.

For any given $\mmy\in\cc{B}$, the {\sc Oracle} finds $\mmx = \argmax_{\mmx\in\cc{A}} \brmf(\mmx)\bdiamond\mmy$.
Let $\mmx = (\mmz, \mmv_1, \dots, \mmv_n, r)\in \bU$ and $\mmy = \cproduct_{i=1}^n (\bar{\mmy}_i, y_{i,0})\in\bV$, the problem can be formatted as:
\beq\label{oldeq:sib_box_oracle}
\begin{aligned}
    \underset{\mmz, \mmq_1, \dots, \mmq_n, r}{\rm maximize}\quad & \big(\sum_{i=1}^n \bar{\mmy}_i \big)^T \mmz - \sum_{i=1}^n \bar{\mmy}_i^T \mmv_i + \big(\sum_{i=1}^n y_{i,0}\big)r\\
    {\rm subject\ to}\quad & \mmz\in\conv(\{\Omega_i\}_{i=1}^n),\\  
    & \mm{\ell}_i \le \mmv_i \le \mmu_i,\ \forall i \in [n],\\
    & r\le \hat{r}.
\end{aligned}
\eeq
Observe that the constraints on $\mmz$, each $\mmv_i$, and $r$ are independent. The problem can be decomposed into smaller problems and be solved individually. 
For each $\mmv_i$, the problem is minimizing a linear function over an AABB, which can be done by identifying the sign of the coefficients. For $j=1,\dots,d$, if $\bar{y}_{i,j} > 0$ we set $v_{i,j} = \ell_{i,j}$ and otherwise $v_{i,j} = u_{i,j}$.
As for $\mmz$, the problem is optimizing a linear function over the convex hull of a set of AABBs.
Since the optimal set contains an extreme point of the convex hull (a vertex of one of the AABBs), the problem can be reduced to the problem of optimizing the linear function over each of the AABBs, which is solvable using the same approach as for $\mmv_i$. For $r$, the optimum is always achieved at $r = \hat{r}$.

Let $(\mmz, \mmv_1, \dots, \mmv_n, r)$ be the output of the {\sc Oracle}.
The width $\rho$ is an upperbound on the spectral norm of $\cproduct_{i=1}^n (\mmz - \mmv_i, r)$ over all possible inputs $\mmy\in\cc{B}$. Since $\mmv_i$ is a point in $\Omega_i$ and also $\conv(\{\Omega_i\}_{i=1}^n)$, we have $\|\mmz - \mmv_i\| \le D,\ \forall i \in [n]$. Consequently,
\[\begin{aligned}
    \Big\|\cproduct_{i=1}^n (\mmz - \mmv_i, r)\Big\|_\spe 
    &= \max_{k\in [2n]}\ \Big|\lambda_{k}\big(\cproduct_{i=1}^n (\mmz - \mmv_i, r)\big) \Big| \\
    &\le \max_{i\in [n]}\ \|\mmz - \mmv_i\| + r\\
    &\le 2D.
\end{aligned}\]
For the last inequality, we used the fact that $r \le \hat{r} \le D$. Therefore, the {\sc Oracle} has a width of $2D$.
By our assumption that $\eps \le {4D \over \hat{r}}$, the additive error $\eps\hat{r}/\sqrt{2}$ is at most $2\rho$ thus satisfies the condition in Theorem~\ref{thm:zero-sum_game}. The total number of iterations for approximating the zero-sum game
is $T = \lceil{32D^2 \ln(2n) \over \eps^2 \hat{r}^2}\rceil$. In each iteration, the algorithm calls the {\sc Oracle} and performs~\eqref{eq:game_update}, which takes $O(nd)$ time.
\end{proof}

Let $\mmv_i = (\mm{\ell}_i + \mmu_i) / 2,\ i = 1,\dots, n$, and let $E = \max_{i\in [n]} \|\mmv_i - \mmv_1\|$. It is clear that the ball $B(\mmv_1, E)$ intersects every AABB. Thus $E$ is an upperbound on the optimal radius $r^*$. Moreover, we have $E \le D \le \rho$. Therefore, the problem of approximately solving~\eqref{eq:sib_box_problem} can be reduced to the problem of solving a sequence of FTPs using the method introduced in Corollary~\ref{coro:sib_cvx_optimization}.

\begin{corollary}
Let $D$ be the diameter of the convex hull $\conv(\{\Omega_i\}_{i=1}^n)$. Let $r^* > 0$ be the optimal value of~\eqref{eq:sib_box_problem} and $R$ be the ratio ${D \over r^*}$. Given an error parameter $\eps > 0$, a $(1+\eps)$-approximate solution of~\eqref{eq:sib_box_problem} can be computed in $O({R^2 nd \log n \over \eps^2})$ time.
\end{corollary}


\subsection{SIB of balls}\label{oldsec:sib_ball}
Let $\Omega_i = B(\mmc_i, r_i),\ i = 1, \dots, n$, be closed balls in the Euclidean space $\bR^d$, where each $\mmc_i \in \bR^d$ and $r_i \ge 0$. Let $B(\mmz, r)$ be a ball in $\bR^d$. Then $B(\mmz, r)$ intersects $B(\mmc_i, r_i)$ if and only if $\|\mmz - \mmc_i\| \le r + r_i$.
The SIB problem for a set of balls can be formatted as the following optimization problem:
\beq\label{oldeq:sib_ball_problem}
\begin{aligned}
    \underset{\mmz, r}{\text{minimize}} \quad &r\\
    \text{subject to}\quad & \| \mmz - \mmc_i \| \le r + r_i,\ \forall i\in [n].\\
\end{aligned}
\eeq

\begin{proposition}
Let $\Omega_i = B(\mmc_i, r_i),\: i = 1, \dots, n$, be closed balls in the Euclidean space $\bR^d$.
\begin{enumerate}
    \item[$(i)$] $B(\mmz, r)$ is a smallest intersecting ball of $\Omega_i$'s if and only if $(\mmz, r)$ is an optimal solution of~\eqref{eq:sib_ball_problem}.
    \item[$(ii)$] Problem~\eqref{eq:sib_ball_problem} is a convex program and a solution always exists.
    \item[$(iii)$] Suppose $\cap_{i=1}^n \Omega_i = \varnothing$. $B(\mmz, r)$ is a smallest intersecting ball of $\Omega_i$'s only if $\mmz\in \conv(\{\mmc_i\}_{i=1}^n)$.
\end{enumerate}
\end{proposition}
\begin{proof}
The proofs of $(i)$ and $(ii)$ are almost identical to the ones in Proposition~\ref{prop:sib_cvx_prop}, thus are omitted here. In what follows, we focus on the justification of $(iii)$.
Let $\cc{D} = \conv(\{\mmc_i\}_{i=1}^n)$. We assume there exists a smallest intersecting ball $B(\mmz, r)$ such that $\mmz\notin \cc{D}$. As $\cap_{i=1}^n \Omega_i = \varnothing$, we know that there exists $i\in [n]$ such that $\|\mmc_i - \mmz\| > 0$, and consequently $r > 0$. 
Let $\mmz' = \Pi(\mmz, \cc{D})$ be the Euclidean projection from $\mmz$ to $\cc{D}$. Thus $\|\mmz - \mmz'\| > 0$. For each $i\in [n]$, we have
\[
    \|\mmc_i - \mmz'\|^2 < \|\mmc_i - \mmz'\|^2 + \|\mmz' - \mmz\|^2 + 2\inprod{\mmc_i - \mmz'}{\mmz' - \mmz} = \|\mmc_i - \mmz\|^2 \le (r + r_i)^2.
\]
The above implies $\|\mmc_i - \mmz'\| < r + r_i,\ \forall i \in [n]$. Let $r' = \max_{i\in [n]} \|\mmc_i - \mmz' \| - r_i$. Then $0 < r' < r$ and the ball $B(\mmz', r')$ intersects all input balls, which is a contradiction.
\end{proof}

Let $r^* > 0$ be the optimal value of problem~\eqref{eq:sib_ball_problem} and $\eps>0$ be an error parameter. We say $(\mmz, r)$ is a $(1+\eps)$-approximate solution of~\eqref{eq:sib_ball_problem} if it is feasible and $r\le (1+\eps)r^*$.
We first consider the FTP:
\begin{flalign}\label{oldeq:sib_ball_ftp}
&\quad
\begin{aligned}
    &\text{\em Given $\hat{r} > 0$, find $\mmz, r$ such that}
\end{aligned}
\quad
\begin{aligned}
    &r \le (1+\eps)\hat{r},\\
    &\|\mmz - \mmc_i\| \le r + r_i, \ \forall i \in [n],\\
    &\mmz \in \conv(\{\mmc_i\}_{i=1}^n).
\end{aligned}
&&
\end{flalign}
Let $D$ be the diameter of the convex hull $\conv(\{\mmc_i\}_{i=1}^n)$. It is clear that $r^* \le D$, then an FTP can be solved using an algorithm that is similar to the one introduced in Theorem~\ref{thm:sib_cvx_thm}.

\begin{theorem}
Let $D$ be the diameter of $\conv(\{\mmc_i\}_{i=1}^n)$ and let $r_{\max} = \max_{i\in [n]} r_i$ be the largest radius of the input balls. 
Given $\hat{r} \in (0, D]$ and an error parameter $\eps\in (0, {4D + 2r_{\max} \over \hat{r}}]$, 
there is an iterative algorithm that solves the feasibility test problem~\eqref{eq:sib_ball_ftp} in $O({(D + r_{\max})^2 \log n \over \eps^2\hat{r}^2})$ iterations, with a processing time of $O(nd)$ per iteration.
\end{theorem}
\begin{proof}
Let $\bU = \bR^d \times \bR$, and let $\brmf: \bU \rightarrow \bV$ be a linear map defined as:
\[
    \brmf(\mmz, r) = \cproduct_{i=1}^n (\mmz - \mmc_i, r + r_i).
\]
Then $(\mmz, r)$ is a feasible solution of~\eqref{eq:sib_ball_problem} only if $\brmf(\mmz, r) \bdiamond \mmy \ge 0, \ \forall \mmy \in \cc{B}$. Define the convex set
\[
    \cc{A} = \Big\{ (\mmz, r) \in \bU : \mmz \in \conv(\{\mmc_i\}_{i=1}^n),\ r \le \hat{r} \Big\}.
\]
Then $\hat{r} \ge r^*$ only if the value $\lambda^*$ of the zero-sum game with $\brmf$ and $\cc{A}$ defined as above is nonnegative. Assume an {\sc Oracle} with width $\rho$. We employ the algorithm described in Theorem~\ref{thm:zero-sum_game} to solve the zero-sum game up to an additive error $\eps\hat{r} / \sqrt{2}$. If there is a certain round $t$ such that $\max_{\mmx \in \cc{A}} \brmf(\mmx) \bdiamond \xt{\mmy}{t} < 0$, we conclude that $\lambda^* < 0$ and $\hat{r} < r^*$.
Conversely, if we have $\brmf(\xt{\mmx}{t})\bdiamond \xt{\mmy}{t} \ge 0$ for all $t = 1, \dots, T$, then $\sum_{t=1}^T \brmf(\xt{\mmx}{t})\bdiamond \xt{\mmy}{t} \ge 0$ and inequality~\eqref{eq:zero-sum_game_eigenvalue} implies $\lambda_{\min}\big(\brmf(\tilde{\mmx})\big) + \eps\hat{r} / \sqrt{2} \ge 0$. 
Let $\tilde{\mmx} = (\tilde{\mmz}, \tilde{r})$. Then $\brmf(\tilde{\mmx}) = \cproduct_{i=1}^n (\tilde{\mmz} - {\mmc}_i, \tilde{r} + r_i)$ and 
\[\begin{aligned}
    \lambda_{\min}\big(\cproduct_{i=1}^n (\tilde{\mmz} - {\mmc}_i, \tilde{r} + r_i) \big) + {\eps \hat{r} \over \sqrt{2}} \ge 0 
    \ \Longrightarrow \ 
    \cproduct_{i=1}^n (\tilde{\mmz} - {\mmc}_i, \tilde{r} + r_i) + {\eps \hat{r} \over \sqrt{2}} \mme \in \cc{C}
    \ \Longrightarrow \ 
    \cproduct_{i=1}^n (\tilde{\mmz} - {\mmc}_i, \tilde{r} + \eps\hat{r} + r_i) \in \cc{C}.
\end{aligned}\]
Since $\tilde{r} + \eps\hat{r} \le (1 + \eps)\hat{r}$, we conclude that $(\tilde{\mmz}, \tilde{r})$ is a feasible solution of~\eqref{eq:sib_ball_problem} with objective value at most $(1+\eps) \hat{r}$.

Let $\mmy = \cproduct_{i=1}^n (\bar{\mmy}_i, y_{i,0})\in \cc{B}$, the {\sc Oracle} solves the following problem:
\beq\label{oldeq:sib_ball_oracle}
\begin{aligned}
    \underset{\mmz, r}{\rm maximize}\quad & \big(\sum_{i=1}^n \bar{\mmy}_i \big)^T \mmz - \sum_{i=1}^n \bar{\mmy}_i^T \mmc_i + \big(\sum_{i=1}^n y_{i,0}\big)r  + \sum_{i=1}^n y_{i,0} r_i\\
    {\rm subject\ to}\quad & \mmz\in\conv(\{\mmc_i\}_{i=1}^n),\\  
    & r\le \hat{r}.
\end{aligned}
\eeq
Observe that the constraints on $\mmz$ and $r$ are independent, and the second and the last term in the objective function are constants. 
The problem can be decomposed into two sub-problems and solved individually. 
For $\mmz$, the problem is optimizing a linear function over the convex hull of a point set. In Theorem~\ref{thm:sib_cvx_thm}, we saw that this problem can be solved by computing the function value at each $\mmc_i$.
For $r$, the optimum is always  $r = \hat{r}$.

Let $(\mmz, r)$ be the output of the above {\sc Oracle}.
The width $\rho$ is an upperbound on the spectral norm of $\cproduct_{i=1}^n (\mmz - \mmc_i, r + r_i)$ over all possible inputs $\mmy\in\cc{B}$. We have
\[\begin{aligned}
    \Big\|\cproduct_{i=1}^n (\mmz - \mmc_i, r + r_i)\Big\|_\spe 
    &= \max_{k\in [2n]}\ \Big|\lambda_{k}\big(\cproduct_{i=1}^n (\mmz - \mmc_i, r + r_i)\big) \Big| \\
    &\le \max_{i\in [n]}\ \|\mmz - \mmc_i\| + r + r_i\\
    &\le 2D + r_{\max}.
\end{aligned}\]
For the last inequality, we used the fact that $r \le \hat{r} \le D$. Therefore, the {\sc Oracle} has a width of $2D + r_{\max}$.
From our assumption that $\eps \le {4D + 2r_{\max} \over \hat{r}}$, the additive error $\eps\hat{r}/\sqrt{2}$ is at most $2\rho$ thus satisfies the condition of Theorem~\ref{thm:zero-sum_game}. The total number of iterations for approximating the zero-sum game
is $T = \lceil{8 (2D + r_{\max})^2 \ln(2n)  \over \eps^2 \hat{r}^2}\rceil$. In each iteration, the algorithm calls the {\sc Oracle} and performs~\eqref{eq:game_update}, which takes $O(nd)$ time.
\end{proof}

Let $E = \max_{i\in [n]} \|\mmc_i - \mmc_1\|$. It is clear that the ball $B(\mmc_1, E)$ intersects every input ball. Thus $E$ is an upperbound on the optimal radius $r^*$. Moreover, we have $E \le D \le \rho$. Therefore, the problem of approximately solving~\eqref{eq:sib_ball_problem} can be reduced to the problem of solving a sequence of FTPs using the method in Corollary~\ref{coro:sib_cvx_optimization}.

\begin{corollary}
Let $D$ be the diameter of $\conv(\{\mmc_i\}_{i=1}^n)$, $r_{\max}$ be the largest radius of the input balls. Let $r^* > 0$ be the optimal value of~\eqref{eq:sib_ball_problem} and $R$ be the ratio ${D + r_{\max} \over r^*}$. Given an error parameter $\eps > 0$, a $(1+\eps)$-approximate solution of~\eqref{eq:sib_ball_problem} can be computed in $O({R^2 nd \log n \over \eps^2})$ time.
\end{corollary}



\subsection{SIB of ellipsoids}\label{oldsec:sib_ellipsoid}
Given a point $\mmc \in \bR^d$ and a symmetric and positive-definite matrix $\mmQ\in \bR^{d\times d}$, we use $\cc{E}(\mmc, \mmQ)$ to denote the ellipsoid $\{\mmv \in \bR^d : (\mmv - \mmc)^T \mmQ (\mmv - \mmc) \le 1\}$.
Let $\Omega_i = \cc{E}(\mmc_i, \mmQ_i),\ i = 1,\dots, n$, be ellipsoids in the Euclidean space $\bR^d$, where $\mmc_i \in \bR^d$ and $\mmQ_i$ is symmetric and positive-definite matrix in $\bR^{d\times d}$.
Then $B(\mmz, r)$ intersects $\cc{E}(\mmc_i, \mmQ_i)$ if and only if there exists $\mmv_i \in \cc{E}(\mmc_i, \mmQ_i)$ such that $\|\mmz - \mmv_i\| \le r$.
We model the SIB problem for a set of ellipsoids as the following optimization problem:
\beq\label{oldeq:sib_ellipsoid_problem}
\begin{aligned}
\underset{\mmz,\mmv_1, \dots, \mmv_n, r}{\rm minimize}\quad & r\\
{\rm subject\ to}\quad & \|\mmz - \mmv_i\| \le r,\ \forall i \in [n],\\
& (\mmv_i - \mmc_i)^T \mmQ_i (\mmv_i - \mmc_i) \le 1,\ \forall i \in [n].
\end{aligned}
\eeq

\begin{proposition}\label{oldprop:sib_ellipsoid_prop}
Let $\Omega_i = \cc{E}(\mmc_i, \mmQ_i)$, $i=1,\dots, n$, be ellipsoids in the Euclidean space $\bR^d$.
\begin{enumerate}
    \item[$(i)$] $B(\mmz, r)$ is a smallest intersecting ball of $\Omega_i$'s if and only if there exists $(\mmv_1, \dots, \mmv_n)$ such that $(\mmz, \mmv_1, \dots, \mmv_n, r)$ is an optimal solution of~\eqref{eq:sib_ellipsoid_problem}.
    \item[$(ii)$] Problem~\eqref{eq:sib_ellipsoid_problem} is a convex program and a solution always exists.
    \item[$(iii)$] $B(\mmz, r)$ is a smallest intersecting ball of $\Omega_i$'s only if $\mmz \in \conv(\{\Omega_i\}_{i=1}^n)$.
\end{enumerate}
\end{proposition}

The proof of Proposition~\ref{prop:sib_ellipsoid_prop} is almost identical to Proposition~\ref{prop:sib_cvx_prop} so is omitted here.
Let $r^* > 0$ be the optimal value of problem~\eqref{eq:sib_ellipsoid_problem} and $\eps>0$ be an error parameter. We say $(\mmz, \mmv_1, \dots, \mmv_n, r)$ is a $(1+\eps)$-approximate solution of~\eqref{eq:sib_ellipsoid_problem} if it is feasible and $r\le (1+\eps)r^*$.
Consider the FTP as follows: 
\begin{flalign}\label{oldeq:sib_ellipsoid_ftp}
&\quad
\begin{aligned}
    &\text{\em Given $\hat{r} > 0$, find $\mmz, r$ such that}
\end{aligned}
\quad
\begin{aligned}
    &r \le (1+\eps)\hat{r},\\
    &\|\mmz - \mmv_i\| \le r, \ \forall i \in [n],\\
    &\mmv_i \in \cc{E}(\mmc_i, \mmQ_i), \ \forall i \in [n],\\
    &\mmz \in \conv(\{\Omega_i\}_{i=1}^n).
\end{aligned}
&&
\end{flalign}
Let $D$ be the diameter of the convex hull $\conv(\{\Omega_i\}_{i=1}^n)$. Clearly, $r^* \le D$, then an FTP can be solved using an algorithm that is similar to the one introduced in Theorem~\ref{thm:sib_cvx_thm}.

\begin{theorem}\label{oldthm:sib_ellipsoid}
Let $D$ be the diameter of $\conv(\{\Omega_i\}_{i=1}^n)$. Given $\hat{r} \in (0, D]$ and an error parameter $\eps\in (0, {4 D \over \hat{r}}]$, there is an iterative algorithm that solves the feasibility test problem~\eqref{eq:sib_ellipsoid_ftp} in $O({D^2 \log n \over \eps^2\hat{r}^2})$ iterations, with $O(nd^2)$ cost per iteration, assuming that the inverses $\mmQ_i^{-1}$ are provided.
\end{theorem}
\begin{proof}
Let $\bU = \bR^d \times \bR^d \times \dots \times \bR^d \times \bR$, and let $\brmf: \bU \rightarrow \bV$ be a linear map defined as:
\[
    \brmf(\mmz, \mmv_1, \dots, \mmv_n, r) = \cproduct_{i=1}^n (\mmz - \mmv_i, r).
\]
Then $(\mmz, \mmv_1, \dots, \mmv_n, r)$ is a feasible solution of~\eqref{eq:sib_ellipsoid_problem} only if $\brmf(\mmz, \mmv_1, \dots, \mmv_n, r) \bdiamond \mmy \ge 0, \ \forall \mmy \in \cc{B}$. Define
\[
    \cc{A} = \Big\{ (\mmz, \mmv_1, \dots, \mmv_n, r) \in \bU : 
    \mmz \in \conv(\{\Omega_i\}_{i=1}^n),\ 
    \mmv_i \in \cc{E}(\mmc_i, \mmQ_i), \forall i \in [n], \
    r \le \hat{r} \Big\}.
\]
Then $\hat{r} \ge r^*$ only if the value $\lambda^*$ of the zero-sum game with $\brmf$ and $\cc{A}$ defined as above is nonnegative. Assume an {\sc Oracle} with width $\rho$. We employ the algorithm described in Theorem~\ref{thm:zero-sum_game} to solve the zero-sum game up to an additive error $\eps\hat{r} / \sqrt{2}$. If there is a certain round $t$ such that $\max_{\mmx \in \cc{A}} \brmf(\mmx) \bdiamond \xt{\mmy}{t} < 0$, we conclude that $\lambda^* < 0$ and $\hat{r} < r^*$.
Conversely, if we have $\brmf(\xt{\mmx}{t})\bdiamond \xt{\mmy}{t} \ge 0$ for all $t = 1, \dots, T$, then $\sum_{t=1}^T \brmf(\xt{\mmx}{t})\bdiamond \xt{\mmy}{t} \ge 0$ and inequality~\eqref{eq:zero-sum_game_eigenvalue} implies $\lambda_{\min}\big(\brmf(\tilde{\mmx})\big) + \eps\hat{r} / \sqrt{2} \ge 0$. 
Let $\tilde{\mmx} = (\tilde{\mmz}, \tilde{\mmv}_1, \dots, \tilde{\mmv}_n, \tilde{r})$. Then $\brmf(\tilde{\mmx}) = \cproduct_{i=1}^n (\tilde{\mmz} - \tilde{\mmv}_i, \tilde{r})$ and 
\[\begin{aligned}
    \lambda_{\min}\big(\cproduct_{i=1}^n (\tilde{\mmz} - \tilde{\mmv}_i, \tilde{r}) \big) + {\eps \hat{r} \over \sqrt{2}} \ge 0 
    \ \Longrightarrow \ 
    \cproduct_{i=1}^n (\tilde{\mmz} - \tilde{\mmv}_i, \tilde{r}) + {\eps \hat{r} \over \sqrt{2}} \mme \in \cc{C}
    \ \Longrightarrow \ 
    \cproduct_{i=1}^n (\tilde{\mmz} - \tilde{\mmv}_i, \tilde{r} + \eps\hat{r}) \in \cc{C}.
\end{aligned}\]
Since $\tilde{r} + \eps\hat{r} \le (1 + \eps)\hat{r}$, we conclude that $(\tilde{\mmz}, \tilde{\mmv}_1, \dots, \tilde{\mmv}_n, \tilde{r})$ is a feasible solution of~\eqref{eq:sib_ellipsoid_problem} with value at most $(1+\eps) \hat{r}$.

Let $\mmy = \cproduct_{i=1}^n (\bar{\mmy}_i, y_{i,0})\in \cc{B}$, the {\sc Oracle} solves the following problem:
\beq\label{oldeq:sib_ellipsoid_oracle}
\begin{aligned}
    \underset{\mmz, \mmv_1, \dots, \mmv_n, r}{\rm maximize}\quad & \big(\sum_{i=1}^n \bar{\mmy}_i \big)^T \mmz - \sum_{i=1}^n \bar{\mmy}_i^T \mmv_i + \big(\sum_{i=1}^n y_{i,0}\big)r\\
    {\rm subject\ to}\quad & \mmz\in\conv(\{\cc{E}(\mmc_1, \mmQ_i)\}_{i=1}^n),\\  
    & \mmv_i \in \cc{E}(\mmc_i, \mmQ_i),\ \forall i \in [n],\\
    & r\le \hat{r}.
\end{aligned}
\eeq
Observe that the constraints on $\mmz$ and $r$ are independent.
The problem can be decomposed into several sub-problems and solved individually. 
For $r$, the optimum is always  $r = \hat{r}$.
For each $\mmv_i$, the problem becomes optimizing a linear function over an ellipsoid. Let $\mmy,\mmc \in \bR^d$ and let $\mmQ\in \bR^{d\times d}$ be a symmetric positive-definite matrix. The problem can be abstracted as:
\beq\label{oldeq:sib_ellipsoid_sub_oracle}
\begin{aligned}
    \underset{\mmv}{\rm maximize} \quad & \mmy^T \mmv \\
    {\rm subject\ to}\quad & (\mmv - \mmc)^T \mmQ (\mmv - \mmc) \le 1.
\end{aligned}
\eeq
The above problem has an analytical solution, where $\mmv = \mmc + {\mmQ^{-1} \mmy \over \sqrt{\mmy^T \mmQ^{-1} \mmy}}$. Therefore, assuming the inverses $\mmQ_i^{-1}$ are pre-computed, the solution for each $\mmv_i$ in~\eqref{eq:sib_ellipsoid_oracle} can be computed in $O(d^2)$ time. 
For $\mmz$, the problem of solving~\eqref{eq:sib_ellipsoid_oracle} is optimizing a linear function over the convex hull of a set of ellipsoids, which can be reduced to solving a sequence of problems in the form of~\eqref{eq:sib_ellipsoid_sub_oracle}.

The analysis on the width of the {\sc Oracle} is identical to Theorem~\ref{thm:sib_box}.
Let $(\mmz, \mmv_1, \dots, \mmv_n, r)$ be the output of the {\sc Oracle}.
The width $\rho$ is an upperbound on the spectral norm of $\cproduct_{i=1}^n (\mmz - \mmv_i, r)$ over all possible inputs $\mmy\in\cc{B}$. Since $\mmv_i$ is a point in $\Omega_i$ and also $\conv(\{\Omega_i\}_{i=1}^n)$, we have $\|\mmz - \mmv_i\| \le D,\ \forall i \in [n]$. Consequently,
\[\begin{aligned}
    \Big\|\cproduct_{i=1}^n (\mmz - \mmv_i, r)\Big\|_\spe 
    &= \max_{k\in [2n]}\ \Big|\lambda_{k}\big(\cproduct_{i=1}^n (\mmz - \mmv_i, r)\big) \Big| \\
    &\le \max_{i\in [n]}\ \|\mmz - \mmv_i\| + r\\
    &\le 2D.
\end{aligned}\]
For the last inequality, we used the fact that $r \le \hat{r} \le D$. Therefore, the {\sc Oracle} has a width of $2D$.
By our assumption that $\eps \le {4D \over \hat{r}}$, the additive error $\eps\hat{r}/\sqrt{2}$ is at most $2\rho$ thus satisfies the condition in Theorem~\ref{thm:zero-sum_game}. The total number of iterations for approximating the zero-sum game
is $T = \lceil{32D^2 \ln(2n) \over \eps^2 \hat{r}^2}\rceil$. In each iteration, the algorithm calls the {\sc Oracle} and performs~\eqref{eq:game_update}, which takes $O(nd^2)$ time.
\end{proof}

Let $E = \max_{i\in [n]} \|\mmc_i - \mmc_1\|$. Then $B(\mmc_1, E)$ intersects all input ellipsoids, and $E$ is an upperbound on the optimal radius $r^*$. The optimization problem~\eqref{eq:sib_ellipsoid_problem} can be reduced to a sequence of FTPs using the approach introduced in Corollary~\ref{coro:sib_cvx_optimization}. Moreover, since $E \le D \le 2\rho$, it also serves as an initial value for guessing the unknown width $\rho$. With an additional pre-processing time of $O(nd^\omega)$ to compute the inverses of $\mmQ_i^{-1}$, where $\omega$ is the exponent for matrix multiplication, we obtain the following result.

\begin{corollary}
Let $D$ be the diameter of the convex hull $\conv(\{\Omega_i\}_{i=1}^n)$. Let $r^* > 0$ be the optimal value of~\eqref{eq:sib_ellipsoid_problem} and $R$ be the ratio ${D \over r^*}$.
Given an error parameter $\eps > 0$, a $(1+\eps)$-approximate solution of~\eqref{eq:sib_ellipsoid_problem} can be computed in $O({R^2 nd^2 \log n \over \eps^2} + nd^{\omega})$ time.
\end{corollary}







==> paper/soft-margin.tex <==

\subsection{Reduced polytopes}\label{oldsec:sib_rcvx}
Let $\cc{V} = \{\mmv_1, \dots, \mmv_m\}$ be a point set in the Euclidean space $\bR^d$, and let $\nu$ be a parameter in the range $[{1\over m}, 1]$. We define the {\em reduced polytope} generated by $\cc{V}$ and $\nu$ as 
\[
    \redpoly(\cc{V}, \nu) = \Big\{\sum_{j=1}^m q_j \mmv_j : \forall \mmq \in \Delta^{m - 1},\ \mmq \le \nu \Big\}.
\]
Let $\cc{V}_1, \dots, \cc{V}_n, \ n > 1$, be non-empty finite point sets in $\bR^d$, where $\cc{V}_i$ consists of $m_i$ points. Let $\mm{\nu} \in \bR^n$ be a set of parameters satisfying $\nu_i \in [{1\over m_i}, 1],\ \forall i \in [n]$.
For $i = 1,\dots, n$, let $\Omega_i$ be the reduced ploytope $\redpoly(\cc{V}_i, \nu_i)$. We want to find the smallest ball that intersects all reduced polytopes.
Let $\mmV_i$ be the matrix that consists of the coordinates of the points in $\cc{V}_i$.
The problem can be modeled as the following optimization problem:
\beq\label{oldeq:sib_rcvx_problem}
\begin{aligned}
    \underset{\mmz, \mmq_1, \dots, \mmq_n, r}{\text{minimize}} \quad &r\\
    \text{subject to}\quad & \| \mmz - \mmV_i \mmq_i \| \le r,\ \forall i\in [n],\\
    & \mmone^T \mmq_i = 1,\ \forall i \in [n],\\
    & 0\le \mmq_i \le \nu_i,\ \forall i \in [n].
\end{aligned}
\eeq

\begin{proposition}\label{oldprop:sib_rcvx_prop}
Let $\Omega_i, i = 1, \dots, n$, be reduced polytopes in $\bR^d$.
\begin{enumerate}
    \item[$(i)$] $B(\mmz, r)$ is a smallest intersecting ball of $\Omega_i$'s if and only if there exists $(\mmq_1, \dots, \mmq_n)$ such that $(\mmz, \mmq_1, \dots, \mmq_n, r)$ is an optimal solution of problem~\eqref{eq:sib_rcvx_problem}.
    \item[$(ii)$] Problem~\eqref{eq:sib_rcvx_problem} is a convex program and a solution always exists.
    \item[$(iii)$] $B(\mmz, r)$ is a smallest intersecting ball of $\Omega_i$'s only if $\mmz \in \conv(\{\Omega_i\}_{i=1}^n)$.
\end{enumerate}
\end{proposition}

The proof of Proposition~\ref{prop:sib_rcvx_prop} is similar to Proposition~\ref{prop:sib_cvx_prop} so is omitted here.
Let $r^* > 0$ be the optimal value of problem~\eqref{eq:sib_rcvx_problem} and $\eps>0$ be an error parameter. We say $(\mmz, \mmq_1, \dots, \mmq_n, r)$ is a $(1+\eps)$-approximate solution of~\eqref{eq:sib_rcvx_problem} if it is feasible and $r\le (1+\eps)r^*$.
Similar to Section~\ref{sec:sib_cvx}, we first consider the FTP:
\begin{flalign}\label{oldeq:sib_rcvx_ftp}
&\quad
\begin{aligned}
    &\text{\em Given $\hat{r} > 0$, find $\mmz, \mmq_1, \dots, \mmq_n, r$ such that}
\end{aligned}
\quad
\begin{aligned}
    &r \le (1+\eps)\hat{r},\\
    &\|\mmz - \mmV_i \mmq_i\| \le r, \ \forall i \in [n],\\
    &\mmq_i \in \Delta^{m_i - 1},\ \forall i \in [n],\\
    &\mmq_i \le \nu_i, \ \forall i \in [n],\\
    &\mmz \in \conv(\{\Omega_i\}_{i=1}^n).
\end{aligned}
&&
\end{flalign}
Let $D$ be the diameter of the convex hull $\conv(\{\Omega_i\}_{i=1}^n)$. Clearly, $r^* \le D$, then an FTP can be solved using an algorithm that is similar to the one introduced in Theorem~\ref{thm:sib_cvx_thm}.

\begin{theorem}
Let $M = \sum_{i=1}^n m_i$ and let $D$ be the diameter of the convex hull $\conv(\{\Omega_i\}_{i=1}^n)$.
Given $\hat{r} \in (0, D]$ and an error parameter $\eps \in (0, {4 D \over \hat{r}}]$, there is an iterative algorithm that solves the feasibility test problem~\eqref{eq:sib_rcvx_ftp} in $O({D^2\log n \over \eps^2 \hat{r}^2})$ iterations, with a processing time of $O(Md)$ per iteration.
\end{theorem}
\begin{proof}
Let $\bU = \bR^d \times \bR^{m_1} \times \dots \times \bR^{m_n} \times \bR$, and let $\brmf : \bU \rightarrow \bV$ be the linear map:
\[
    \brmf(\mmz, \mmq_1, \dots, \mmq_n, r) = \cproduct_{i=1}^n (\mmz - \mmV_i\mmq_i, r).
\]
Then $(\mmz, \mmq_i, \dots, \mmq_n, r)$ is feasible to~\eqref{eq:sib_rcvx_ftp} only if $\brmf(\mmz, \mmq_1, \dots, \mmq_n, r) \bdiamond \mmy \ge 0,\ \forall \mmy \in \cc{B}$. Define the convex set
\[
    \cc{A} = \Big\{(\mmz, \mmq_1,\dots,\mmq_n, r) \in \bU : \mmz\in\conv(\{\Omega_i\}_{i=1}^n),\ \mmq_i \in \Delta^{m_i - 1}, \mmq_i \le \nu_i, \forall i\in [n],\ r \le \hat{r} \Big\}.
\]
Consequently, $\hat{r} \ge r^*$ only if the value $\lambda^*$ of the zero-sum game with $\brmf$ and $\cc{A}$ defined as above is nonnegative.
Assume an {\sc Oracle} with width $\rho$. Similar to Theorem~\ref{thm:sib_cvx_thm},
we employ the algorithm described in Theorem~\ref{thm:zero-sum_game} to solve the zero-sum game up to an additive error $\eps\hat{r} / \sqrt{2}$.
During the process of this algorithm, if there is certain round $t$ such that $\max_{\mmx\in\cc{A}}\ \brmf(\mmx)\bdiamond\xt{\mmy}{t} < 0$, we terminate the algorithm and conclude that $\hat{r} < r^*$.
Conversely, if we have $\brmf(\xt{\mmx}{t})\bdiamond \xt{\mmy}{t} \ge 0$ for all $t = 1, \dots, T$, then $\sum_{t=1}^T \brmf(\xt{\mmx}{t})\bdiamond \xt{\mmy}{t} \ge 0$ and inequality~\eqref{eq:zero-sum_game_eigenvalue} implies $\lambda_{\min}\big(\brmf(\tilde{\mmx})\big) + \eps\hat{r} / \sqrt{2} \ge 0$. Let $\tilde{\mmx} = (\tilde{\mmz}, \tilde{\mmq}_1, \dots, \tilde{\mmq}_n, \tilde{r})$. Then $\brmf(\tilde{\mmx}) = \cproduct_{i=1}^n (\tilde{\mmz} - \mmV_i \tilde{\mmq}_i, \tilde{r})$ and 
\[\begin{aligned}
    \lambda_{\min}\big(\cproduct_{i=1}^n (\tilde{\mmz} - \mmV_i \tilde{\mmq}_i, \tilde{r}) \big) + {\eps \hat{r} \over \sqrt{2}} \ge 0 
    \ \Longrightarrow \ 
    \cproduct_{i=1}^n (\tilde{\mmz} - \mmV_i \tilde{\mmq}_i, \tilde{r}) + {\eps \hat{r} \over \sqrt{2}} \mme \in \cc{C}
    \ \Longrightarrow \ 
    \cproduct_{i=1}^n (\tilde{\mmz} - \mmV_i \tilde{\mmq}_i, \tilde{r} + \eps\hat{r}) \in \cc{C}.
\end{aligned}\]
Since $(\tilde{\mmz}, \tilde{\mmq}_1, \dots, \tilde{\mmq}_n, \tilde{r} + \eps\hat{r})$ satisfies all the conditions in~\eqref{eq:sib_rcvx_ftp}, we conclude that it is a feasible solution of~\eqref{eq:sib_rcvx_problem} with objective value at most $(1+\eps)\hat{r}$.

Let $\mmy = \cproduct_{i=1}^n (\bar{\mmy}_i, y_{i,0})$ be a point in $\cc{B}$, the {\sc Oracle} needs to solve the following problem:
\beq\label{oldeq:sib_rcvx_oracle}
\begin{aligned}
    \underset{\mmz, \mmq_1, \dots, \mmq_n, r}{\rm maximize}\quad & \big(\sum_{i=1}^n \bar{\mmy}_i \big)^T \mmz - \sum_{i=1}^n (\bar{\mmy}_i^T \mmV_i ) \mmq_i + \big(\sum_{i=1}^n y_{i,0}\big)r\\
    {\rm subject\ to}\quad & \mmz\in\conv(\{\Omega_i\}_{i=1}^n),\\  
    & \mmq_i\in \Delta^{m_i - 1},\ \forall i \in [n],\\
    &\mmq_i \le \nu_i, \ \forall i \in [n],\\
    & r\le \hat{r}.
\end{aligned}
\eeq
The above problem is almost identical to~\eqref{eq:sib_cvx_oracle}, except that here we have an additional upperbound on the values of $\mmq_i$.
Similar to~\eqref{eq:sib_cvx_oracle}, the problem can be decomposed into smaller problems and be solved individually. For $r$, the optimum is $r = \hat{r}$.
For each $\mmq_i$, the problem is minimizing a linear function over a ``reduced simplex''.
Let $\mmc$ be a vector in $\bR^m$ and let $\nu$ be a scalar in the range $[{1\over m}, 1]$. We abstract the problem as:
\beq\label{oldeq:sib_rcvx_oracle_abs}
\begin{aligned}
    \underset{\mmq}{\rm maximize} \quad & \mmc^T \mmq\\
    {\rm subject\ to} \quad & \mmone^T \mmq = 1,\\
    & 0 \le \mmq \le \nu.
\end{aligned}
\eeq
Let $k = \lceil {1\over \nu} \rceil$. The problem can be solved by identifying the $k$ largest entries in $\mmc$. Let $j_1, \dots, j_k$ be the indices of the $k$ largest entries, where $c_{j_1} \ge c_{j_2} \ge \dots \ge c_{j_k}$. Then the optimum is given by
\[
    q_j  =
    \begin{cases}
        \nu, &\text{for $j = j_1, \dots, j_{k-1}$},\\
        1 - \nu(k-1), &\text{for $j = j_k$},\\
        0, &\text{otherwise}.
    \end{cases}
\]
Employing the well-known median-finding algorithms~\cite{???} to find the $k$-th largest entry, problem~\eqref{eq:sib_rcvx_oracle_abs} can be solved in $O(m)$ time. 
Therefore, to solve the {\sc Oracle} program~\eqref{eq:sib_rcvx_oracle} for $\mmq_i$'s, the running time is dominated by the time for computing the coefficient $\bar{\mmy}_i^T \mmV_i$, which is $O(Md)$.
For $\mmz$, the problem is optimizing a linear function over the convex hull of a set of reduced polytopes, which can be solved by optimizing the function over each of the reduced polytopes individually.
The latter is again reduced to a problem in the form of~\eqref{eq:sib_rcvx_oracle_abs}.

Let $(\mmz, \mmq_1, \dots, \mmq_n, r)$ be the output of the above {\sc Oracle}.
The width $\rho$ of the {\sc Oracle} is an upperbound on the spectral norm of $\cproduct_{i=1}^n (\mmz - \mmV_i \mmq_i, r)$ over all possible inputs $\mmy\in\cc{B}$. 
Since the point $\mmV_i\mmq_i$ is in $\Omega_i$ and also $\conv(\{\Omega_i\}_{i=1}^n)$. Consequently, we have $\|\mmz - \mmV_i \mmq_i\| \le D,\ \forall i \in [n]$. Then,
\[\begin{aligned}
    \Big\|\cproduct_{i=1}^n (\mmz - \mmV_i \mmq_i, r)\Big\|_\spe 
    &= \max_{k\in [2n]}\ \Big|\lambda_{k}\big(\cproduct_{i=1}^n (\mmz - \mmV_i \mmq_i, r)\big) \Big| \\
    &\le \max_{i\in [n]}\ \|\mmz - \mmV_i\mmq_i\| + r\\
    &\le 2D.
\end{aligned}\]
For the last inequality, we used the fact that $r \le \hat{r} \le D$. Therefore, the {\sc Oracle} has a width of $2D$.
By our assumption that $\eps \le {4 D \over \hat{r}}$, the additive error $\eps\hat{r}/\sqrt{2}$ is at most $2\rho$ thus satisfies the condition in Theorem~\ref{thm:zero-sum_game}. The total number of iterations for approximating the zero-sum game
is $T = \lceil{32D^2 \ln(2n) \over \eps^2 \hat{r}^2}\rceil$. In each iteration, the algorithm calls the {\sc Oracle} and performs~\eqref{eq:game_update}, which takes $O(Md + nd) = O(Md)$ time.
\end{proof}

For $i = 1,\dots, n$, let $\mmq_i = ({1\over m_i}, \dots, {1\over m_i})$ and let $\mmv_i = \mmV_i \mmq_i$. Then we have $\mmv_i \in \redpoly(\cc{V}_i, \nu_i),\ \forall i \in [n]$. Let $E = \max_{i\in [n]} \|\mmv_i - \mmv_1\|$. It is easily seen that the ball $B(\mmv_1, E)$ intersects all reduced polytopes, so $E$ is an upperbound on the optimal radius $r^*$. Moreover, we have $E \le D \le \rho$. Therefore, the problem of approximately solving~\eqref{eq:sib_rcvx_problem} can be reduced to the problem of solving a sequence of FTPs in the form~\eqref{eq:sib_rcvx_ftp} using a method similar to the one introduced in Corollary~\ref{coro:sib_cvx_optimization}.

\begin{corollary}
Let $M = \sum_{i=1}^n m_i$ and let $D$ be the diameter of the convex hull $\conv(\{\Omega_i\}_{i=1}^n)$.
Let $r^* > 0$ be the optimal value of~\eqref{eq:sib_rcvx_problem} and $R$ be the ratio $D\over r^*$. Given an error parameter $\eps>0$, a $(1+\eps)$-approximate solution of~\eqref{eq:sib_rcvx_problem} can be computed in $O({R^2 Md \log n \over \eps^2})$ time.
\end{corollary}



\subsection{SIB with outliers}\label{oldsec:sib_outlier}
We adopt the idea of soft-margin SVDD to handle the outliers. Let $C>0$ be a user-specified parameter and introduce a slack variable $\xi_i$ for each of the convex polytopes. 
We propose the following variant of the SIB problem:
\beq\label{oldeq:soft_sib_problem}
\begin{aligned}
    \underset{\mmz, \mmq_1, \dots, \mmq_n, \mmxi, r}{\text{minimize}} \quad &r + C\sum_{i=1}^n \xi_i \\
    \text{subject to}\quad & \| \mmz - \mmV_i \mmq_i \| \le r + \xi_i,\ \forall i\in [n],\\
    & \mmone^T \mmq_i = 1,\ \forall i \in [n], \\
    & \mmq_i \ge 0,\ \forall i \in [n],\\
    & \mmxi \ge 0,\: r \ge 0.
\end{aligned}
\eeq

\begin{proposition}\label{oldprop:soft_sib_prop}
Let $\cc{V}_i, i = 1, \dots, n$, be point sets in $\bR^d$, and let $\Omega_i = \conv(\cc{V}_i), \forall i \in [n]$.
\begin{enumerate}
\item[$(i)$] Problem~\eqref{eq:soft_sib_problem} is a convex program and a solution always exists.
\item[$(ii)$] If $C > 1$, then any optimal solution of problem~\eqref{eq:soft_sib_problem} has $\mmxi = 0$.
\item[$(iii)$] If $C < {1\over n}$, then any optimal solution of problem~\eqref{eq:soft_sib_problem} has $r = 0$. 
\item[$(iv)$] Problem~\eqref{eq:soft_sib_problem} has an optimal solution with $\mmz\in \conv(\{\Omega_i\}_{i=1}^n)$. 
\end{enumerate}
\end{proposition}

\begin{proof}
$(i)$
The problem is a convex program because the objective function is linear and all the constraints are convex constraints.
To see the existence of a solution,
let $(\mmz, \mmq_1, \dots, \mmq_n, r)$ be a solution of problem~\eqref{eq:sib_cvx_problem}. Then $(\mmz, \mmq_1, \dots, \mmq_n, \mmzero, r)$ must be a feasible solution of~\eqref{eq:soft_sib_problem}.

$(ii)$
Let $(\mmz, \mmq_1, \dots, \mmq_n, \mmxi, r)$ be any solution with $\mmxi \ne 0$. Let $\xi_{\max} = \max_{i\in [n]} \xi_i$.
Then,
\[\begin{aligned}
    & r + \xi_{\max} < r + C\xi_{\max} \le r + C \sum_{i = 1}^n \xi_i,\\
    & \|\mmz - \mmV_i \mmq_i\| \le r + \xi_{\max}, \ \forall i \in [n],
\end{aligned}\]
which implies $(\mmz, \mmq_1, \dots, \mmq_n, \mmzero, r + \xi_{\max})$ is a feasible solution of~\eqref{eq:soft_sib_problem} with a smaller objective value.

$(iii)$
Let $(\mmz, \mmq_1, \dots, \mmq_n, \mmxi, r)$ be any solution with $r > 0$. Then,
\[\begin{aligned}
    & C \sum_{i=1}^n (\xi_i + r) = C n r + C\sum_{i=1}^n \xi_i < r + C\sum_{i=1}^n \xi_i,\\
    & \|\mmz - \mmV_i \mmq_i \| \le \xi_i + r, \ \forall i \in [n],
\end{aligned}\]
which implies $(\mmz, \mmq_1, \dots, \mmq_1, \mmxi + r, 0)$ is a feasible solution of~\eqref{eq:soft_sib_problem} with a smaller objective value.

$(iv)$
Let $\cc{D}$ be the convex hull $\conv(\{\Omega_i\}_{i=1}^n)$.
Let $(\mmz, \mmq_1, \dots, \mmq_n, \mmxi, r)$ be any optimal solution with $\mmz \notin \cc{D}$. Let $\mmz' = \Pi(\mmz, \cc{D})$, so $\|\mmz - \mmz'\| > 0$. For $i = 1,\dots,n$, let $\mmv_i = \mmV_i \mmq_i$. By the projection theorem, we have
\[
    \|\mmz' - \mmv_i\| < \|\mmz - \mmv_i\| \le r + \xi_i, \ \forall i \in [n].
\]
Let $\alpha = \max_{i\in [n]} \|\mmz' - \mmv_i\| - \xi_i$ and let $r' = \max\{0, \alpha\}$. Then $(\mmz', \mmq_1, \dots, \mmq_n, \mmxi, r')$ is a feasible solution of~\eqref{eq:soft_sib_problem} with objective value at most $r + C \sum_{i=1}^n \xi_i$. Since $r + C \sum_{i=1}^n \xi_i$ is the optimal value, $(\mmz', \mmq_1, \dots, \mmq_n, \mmxi, r')$ is an optimal solution with $\mmz' \in \cc{D}$.
\end{proof}

Let $\alpha^* > 0$ be the optimal value of problem~\eqref{eq:sib_rcvx_problem} and $\eps>0$ be an error parameter. We say $(\mmz, \mmq_1, \dots, \mmq_n, \mmxi, r)$ is a $(1+\eps)$-approximate solution of~\eqref{eq:soft_sib_problem} if it is feasible and $r + C\sum_{i=1}^n \xi_i \le (1+\eps)\alpha^*$.
We consider an FTP that is slightly different from before:
\begin{flalign}\label{oldeq:soft_sib_ftp}
&\quad
\begin{aligned}
    &\text{\em Given $\hat{\alpha} > 0$, find $\mmz, \mmq_1, \dots, \mmq_n, \mmxi, r$ such that}
\end{aligned}
\quad
\begin{aligned}
    &r + C\sum_{i=1}^n \xi_i \le (1+\eps)\hat{\alpha},\\
    &\|\mmz - \mmV_i \mmq_i\| \le r + \xi_i, \ \forall i \in [n],\\
    &\mmq_i \in \Delta^{m_i - 1},\ \forall i \in [n],\\
    &\mmxi \ge 0,\ r \ge 0,\\
    &\mmz \in \conv(\{\Omega_i\}_{i=1}^n).
\end{aligned}
&&
\end{flalign}
Let $D$ be the diameter of the convex hull $\conv(\{\Omega\}_{i=1}^n)$.
Since any solution of~\eqref{eq:sib_cvx_problem} implies a solution of~\eqref{eq:soft_sib_problem} with the same objective value (by setting $\mmxi = 0$), $D$ is an upperbound on the optimum $\alpha^*$. An FTP in the form of~\eqref{eq:soft_sib_problem} can also be solved via approximating the zero-sum game.

\begin{theorem}
Let $M = \sum_{i=1}^n m_i$ and let $D$ be the diameter of the convex hull $\conv(\{\Omega_i\}_{i=1}^n)$.
Given $\hat{\alpha} \in (0, D]$ and an error parameter $\eps \in (0, {4 D \over C\hat{\alpha}}]$, there is an iterative algorithm that solves the feasibility test problem~\eqref{eq:soft_sib_ftp} in $O({D^2\log n \over C^2 \eps^2 \hat{\alpha}^2})$ iterations, with a processing time of $O(Md)$ per iteration.    
\end{theorem}
\begin{proof}
Let $\bU = \bR^d \times \bR^{m_1} \times \dots \times \bR^{m_n} \times \bR^n \times \bR$, and let $\brmf : \bU \rightarrow \bV$ be the linear map:
\[
    \brmf(\mmz, \mmq_1, \dots, \mmq_n, \mmxi, r) = \cproduct_{i=1}^n (\mmz - \mmV_i\mmq_i, r + \xi_i).
\]
Then $(\mmz, \mmq_i, \dots, \mmq_n, \mmxi, r)$ is feasible to~\eqref{eq:sib_rcvx_ftp} only if $\brmf(\mmz, \mmq_1, \dots, \mmq_n, \mmxi, r) \bdiamond \mmy \ge 0,\ \forall \mmy \in \cc{B}$. Define the convex set
\[\begin{aligned}
    \cc{A} = \Big\{(\mmz, \mmq_1,\dots,\mmq_n, \mmxi, r) \in \bU : \mmz\in\conv(\{\Omega_i\}_{i=1}^n),\ \mmq_i \in \Delta^{m_i - 1}, \forall i\in [n],\ r + C\sum_{i=1}^n \xi_i \le \hat{\alpha},\ \mmxi \ge 0,\ r\ge 0 \Big\}.
\end{aligned}
\]
Let $\cc{O}^*$ be the set of optimal solutions of~\eqref{eq:soft_sib_problem}. Then for any $\mmx \in \cc{O}^*$ and $\mmy\in \cc{B}$ we have $\brmf(\mmx)\bdiamond \mmy \ge 0$. From Proposition~\ref{prop:soft_sib_prop}, we know that if $\hat{\alpha} \ge \alpha^*$, then $\cc{O}^*\cap \cc{A} \neq \varnothing$. Consequently, the value $\lambda^*$ of the zero-sum game with $\brmf$ and $\cc{A}$ defined as above is nonnegative.
Assume an {\sc Oracle} with width $\rho$. We employ the algorithm in Theorem~\ref{thm:zero-sum_game} to solve the zero-sum game up to an additive error $\eps\hat{\alpha} / \sqrt{2}$.
During the process of this algorithm, if there is certain round $t$ such that $\max_{\mmx\in\cc{A}}\ \brmf(\mmx)\bdiamond\xt{\mmy}{t} < 0$, we terminate the algorithm and conclude that $\hat{\alpha} < \alpha^*$.
Conversely, if we have $\brmf(\xt{\mmx}{t})\bdiamond \xt{\mmy}{t} \ge 0$ for all $t = 1, \dots, T$, then $\sum_{t=1}^T \brmf(\xt{\mmx}{t})\bdiamond \xt{\mmy}{t} \ge 0$ and inequality~\eqref{eq:zero-sum_game_eigenvalue} implies $\lambda_{\min}\big(\brmf(\tilde{\mmx})\big) + \eps\hat{\alpha} / \sqrt{2} \ge 0$. Let $\tilde{\mmx} = (\tilde{\mmz}, \tilde{\mmq}_1, \dots, \tilde{\mmq}_n, \tilde{\mmxi}, \tilde{r})$. Then $\brmf(\tilde{\mmx}) = \cproduct_{i=1}^n (\tilde{\mmz} - \mmV_i \tilde{\mmq}_i, \tilde{r} + \tilde{\xi}_i)$ and 
\[\begin{aligned}
    \lambda_{\min}\big(\cproduct_{i=1}^n (\tilde{\mmz} - \mmV_i \tilde{\mmq}_i, \tilde{r} + \tilde{\xi}_i) \big) + {\eps \hat{\alpha} \over \sqrt{2}} \ge 0 
    \ \Longrightarrow \ 
    \cproduct_{i=1}^n (\tilde{\mmz} - \mmV_i \tilde{\mmq}_i, \tilde{r} + \tilde{\xi}_i) + {\eps \hat{\alpha} \over \sqrt{2}} \mme \in \cc{C}
    \ \Longrightarrow \ 
    \cproduct_{i=1}^n (\tilde{\mmz} - \mmV_i \tilde{\mmq}_i, \tilde{r} + \tilde{\xi}_i + \eps\hat{\alpha}) \in \cc{C}.
\end{aligned}\]
Consequently, we see that $(\tilde{\mmz}, \tilde{\mmq}_1, \dots, \tilde{\mmq}_n, \tilde{\mmxi}, \tilde{r} + \eps\hat{\alpha})$ satisfies all the conditions in~\eqref{eq:soft_sib_ftp} and is a feasible solution of~\eqref{eq:soft_sib_problem} with objective value at most $(1+\eps)\hat{\alpha}$.

Given any point $\mmy\in\cc{B}$, the {\sc Oracle} finds $\mmx = \argmax_{\mmx\in\cc{A}} \brmf(\mmx)\bdiamond\mmy$.
Let $\mmx = (\mmz, \mmq_1, \dots, \mmq_n, \mmxi, r)\in \bU$ and $\mmy = \cproduct_{i=1}^n (\bar{\mmy}_i, y_{i,0})\in\bV$, the problem can be formatted as:
\beq\label{oldeq:soft_sib_oracle}
\begin{aligned}
    \underset{\mmz, \mmq_1, \dots, \mmq_n, \mmxi, r}{\rm maximize}\quad & \big(\sum_{i=1}^n \bar{\mmy}_i \big)^T \mmz - \sum_{i=1}^n (\bar{\mmy}_i^T \mmV_i ) \mmq_i + \big(\sum_{i=1}^n y_{i,0}\big)r + \sum_{i=1}^n y_{i,0}\xi_i\\
    {\rm subject\ to}\quad & \mmz\in\conv(\{\Omega_i\}_{i=1}^n),\\  
    & \mmq_i\in \Delta^{m_i - 1},\ \forall i \in [n],\\
    & r + C \sum_{i=1}^n \xi_i \le \hat{\alpha},\\
    & \mmxi \ge 0,\ r \ge 0.
\end{aligned}
\eeq
Observe that for $\mmz$ and each $\mmq_i$, the objectives and constraints are independent of the other variables. The solutions for $\mmz$ and each $\mmq_i$ are identical to~\eqref{eq:sib_cvx_oracle}. For $\mmxi$ and $r$, the problem can be simplified to the following:
\beq\label{oldeq:soft_sib_oracle_simple}
\begin{aligned}
    \underset{\mmxi, r}{\rm maximize}\quad & {1\over \sqrt{2}}r + \sum_{i=1}^n y_{i,0}\xi_i\\
    {\rm subject\ to}\quad &  r + C \sum_{i=1}^n \xi_i \le \hat{\alpha},\\
    & \mmxi \ge 0,\ r \ge 0.
\end{aligned}
\eeq
The above problem is optimizing a linear function over the intersection of a halfspace and the nonnegative orthant. To solve this problem, we can compute the function value at each of the extreme points of the feasible region, and take the maximum therein.
The extreme points of the region (except the origin) are given by $(\mmzero, \hat{\alpha})$ and $({\hat{\alpha}\over C }\mme_i, 0)$, $\forall i \in [n]$, where $\mme_i$ is the $i$-th unit vector, and the function values at which are ${\hat{\alpha} \over \sqrt{2}}$ and ${y_{i,0} \hat{\alpha} \over C}$ respectively.
Let $i^* = \argmax_{i\in [n]} y_{i,0}$. The solution of~\eqref{eq:soft_sib_oracle_simple} is:
\[
    r = \begin{cases}
        \hat{\alpha} & \text{if ${y_{i^*,0} \over C} \le {1\over \sqrt{2}}$,}\\
        0 & \text{otherwise,}
    \end{cases} \quad
    \xi_{i^*} = \begin{cases}
        0 & \text{if ${y_{i^*,0} \over C} \le {1\over \sqrt{2}}$,}\\
        {y_{i^*,0} \hat{\alpha} \over C} & \text{otherwise,}
    \end{cases} \quad 
    \xi_i = 0 \ \text{for $i\ne i^*$.}
\]

Let $(\mmz, \mmq_1, \dots, \mmq_n, \mmxi, r)$ be the output of the above {\sc Oracle}.
The width $\rho$ of the {\sc Oracle} is an upperbound on the spectral norm of $\cproduct_{i=1}^n (\mmz - \mmV_i \mmq_i, r + \xi_i)$ over all possible inputs $\mmy\in\cc{B}$. 
Since the point $\mmV_i\mmq_i$ is in $\Omega_i$ and also $\conv(\{\Omega_i\}_{i=1}^n)$. Consequently, we have $\|\mmz - \mmV_i \mmq_i\| \le D,\ \forall i \in [n]$. Then,
\[\begin{aligned}
    \Big\|\cproduct_{i=1}^n (\mmz - \mmV_i \mmq_i, r + \xi_i)\Big\|_\spe 
    &= \max_{k\in [2n]}\ \Big|\lambda_{k}\big(\cproduct_{i=1}^n (\mmz - \mmV_i \mmq_i, r + \xi_i)\big) \Big| \\
    &\le \max_{i\in [n]}\ \|\mmz - \mmV_i\mmq_i\| + r + \xi_i\\
    &\overset{(a)}{\le} D + \max\{\hat{\alpha}, {\hat{\alpha} \over \sqrt{2} C} \} \\
    &\overset{(b)}{\le} D + \max\{D, {D \over \sqrt{2}C} \}.
\end{aligned}\]
For $(a)$, we used the fact that $y_{i,0}\le {1\over \sqrt{2}}$; and $(b)$ is due to $\hat{\alpha} \le D$. 
Since when $C>1$, problem~\eqref{eq:soft_sib_oracle} is equivalent to~\eqref{eq:sib_cvx_problem} and the {\sc Oracle} always outputs $\mmxi_i = 0$, here we assume $C \le 1$. In which case the above result can be further simplified to $D + \max\{D, {D \over \sqrt{2}C}\} \le {2D \over C}$.
Therefore, if $C \le 1$, the {\sc Oracle} has a width of ${2D \over C}$.
By our assumption that $\eps \le {4 D \over C\hat{\alpha}}$, the additive error $\eps\hat{\alpha}/\sqrt{2}$ is at most $2\rho$ thus satisfies the condition in Theorem~\ref{thm:zero-sum_game}. The total number of iterations for approximating the zero-sum game
is $T = \lceil{32D^2 \ln(2n) \over C^2 \eps^2 \hat{r}^2}\rceil$. In each iteration, the algorithm calls the {\sc Oracle} and performs~\eqref{eq:game_update}, which takes $O(Md)$ time.
\end{proof}

Same as Corollary~\ref{coro:sib_cvx_optimization}, pick a point $\mmv_i$ in each $\cc{V}_i$ and compute $E = \max_{i\in [n]} \|\mmv_i - \mmv_1\|$. Then the quantity $E$ is an upperbound on the optimal value $\alpha^*$. The optimization problem~\eqref{eq:soft_sib_problem} can be reduced to a sequence of FTPs by employing the searching strategy in Corollary~\ref{coro:sib_cvx_optimization} for optimizing $\hat{\alpha}$. Moreover, if $C \le 1$, we have $E \le D \le 2\rho$, and the method for working with unknown width is also applicable.

\begin{corollary}
Let $M = \sum_{i=1}^n m_i$ and let $D$ be the diameter of the convex hull $\conv(\{\Omega_i\}_{i=1}^n)$.
Let $\alpha^* > 0$ be the optimal value of~\eqref{eq:soft_sib_problem} and $R$ be the ratio $D\over \alpha^*$. Given an error parameter $\eps>0$, a $(1+\eps)$-approximate solution of~\eqref{eq:soft_sib_problem} can be computed in $O({R^2 Md \log n \over C^2\eps^2})$ time.
\end{corollary}


==> paper/todelete.tex <==
\section*{New Structure}

\begin{enumerate}
    \item[] Abstract
    \item Introduction
    \item Preliminaries $\checkmark$
    \item Approximate a zero-sum game $\checkmark$
    \item Smallest intersecting ball $\checkmark$
    \begin{enumerate}
        \item General problem $\checkmark$
        \item Convex polytopes $\checkmark$
        \item Reduced polytopes $\checkmark$
        \item Boxes $\checkmark$
        \item Balls $\checkmark$
        \item Ellipsoids $\checkmark$
        \item Extensions $\checkmark$
    \end{enumerate}
    \item Soft-margin variant
    \begin{enumerate}
        \item General problem $\checkmark$
        \item Singletons
    \end{enumerate}
    \item Discussion
    \item[A] SIB, PD and SVM 
\end{enumerate}








\section*{Intro and Discussion}

\begin{itemize}
    \item The convex sets $\Omega_i$ can actually be convex hulls of small convex sets, in which case we obtain an algorithm for solving SVM under uncertainty.
    \item SIB in Hilbert space or using kernel functions
    \item Barycentric coordinate for continuous convex sets
\end{itemize}

